Story Beyond the Eye: Glyph Positions Break PDF Text Redaction

In this work we find that many current redactions of PDF text are insecure due to non-redacted character positioning information. In particular, subpixel-sized horizontal shifts in redacted and non-redacted characters can be recovered and used to effectively deredact first and last names. Unfortunately these findings affect redactions where the text underneath the black box is removed from the PDF. We demonstrate these findings by performing a comprehensive vulnerability assessment of common PDF redaction types. We examine 11 popular PDF redaction tools, including Adobe Acrobat, and find that they leak information about redacted text. We also effectively deredact hundreds of real-world PDF redactions, including those found in OIG investigation reports and FOIA responses. To correct the problem, we have released open source algorithms to fix trivial redactions and reduce the amount of information leaked by nonexcising redactions (where the text underneath the redaction is copy-pastable). We have also notified the developers of the studied redaction tools. We have notified the Office of Inspector General, the Free Law Project, PACER, Adobe, Microsoft, and the US Department of Justice. We are working with several of these groups to prevent our discoveries from being used for malicious purposes.

==> abstract-scrap.tex <==


\begin{abstract}
In the past redaction involved the use of black or white markers or paper cut-outs to obscure content on physical paper. Today many redactions take place on digital PDF documents and redaction is often performed by software tools. Typical redaction tools remove text from PDF documents and draw a black or white rectangle in its place, mimicking a physical redaction. This practice is thought to be secure when the redacted text is removed and cannot be ``copy-pasted'' from the PDF document. We find this common conception is false---existing PDF redactions can be broken by precise measurements of non-redacted character positioning information.

We develop a deredaction tool for automatically finding and breaking these vulnerable redactions. We report on 11 different redaction tools, finding the majority do not remove redaction-breaking information, including some Adobe Acrobat workflows. We empirically measure the information leaks, finding some redactions leak upwards of 15 bits of information, creating a 32,768-fold reduction in the space of potential redacted texts. We demonstrate a lower bound on the impact of these leaks via a 22,120 document study, including 18,975 Office of the Inspector General (OIG) investigation reports, where we find 769 vulnerable named-entity redactions. We find leaked information reduces the contents for 164 of these redacted names to less than 494 possibilities from a 7 million name dictionary. We show these findings impact by breaking redactions from the Epstein/Maxwell case, Manafort case, and a released Snowden document. Moreover, we develop an efficient algorithm for locating copy-pastable redactions and find over 100,000 poorly redacted words in US court documents. Current PDF text redaction methods are insufficient for named entity protection.
\end{abstract}

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002978.10003006.10011608</concept_id>
       <concept_desc>Security and privacy~Information flow control</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002978.10003029.10011150</concept_id>
       <concept_desc>Security and privacy~Privacy protections</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002978.10003029.10003032</concept_id>
       <concept_desc>Security and privacy~Social aspects of security and privacy</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10002978.10003022.10003465</concept_id>
       <concept_desc>Security and privacy~Software reverse engineering</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10002978.10003022.10003023</concept_id>
       <concept_desc>Security and privacy~Software security engineering</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Information flow control}
\ccsdesc[500]{Security and privacy~Privacy protections}
\ccsdesc[500]{Security and privacy~Social aspects of security and privacy}
\ccsdesc[300]{Security and privacy~Software reverse engineering}
\ccsdesc[500]{Security and privacy~Software security engineering}

\keywords{redaction; privacy; information leaks; portable document format; PDF; measurement; law; reverse engineering} % TODO: replace with your keywords


==> acks.tex <==
\section*{Acknowledgments}
\label{sec:acks}

We dedicate this work to Pere Ubu and Richard Terdiman.
While unaffiliated with this work's content, they inspired the clarity and strength required for the project to reach fruition.


==> appdx-safe.tex <==
\appendix
\label{sec:appdx}

\section{Dictionary Construction}
\label{sec:dictdetail}

This paper used several dictionaries.
In order to ensure the quality of the guessed text, we manually sourced and refined the following:

\begin{enumerate}
\item \textit{Word} was sourced from the linux spellchecker: \url{/usr/share/dict/american-english} filtered for pronouns (first letter upper case), stop words sans pronouns, and words containing punctuation and digits. Single quotes were made to be curly possessive and straight to match the document under study.
\item \textit{FN} were sourced from from the US social security agency~\cite{ssaNames} starting from 1880. For both this and the last name dictionary names like ``McCarthy'' were made to be correctly capitalized.
\item \textit{LN} were sourced from the year 2000 US Census~\cite{usCensus}.
\item \textit{Ctry} was sourced from wikipedia lists of countries and alternative country names~\cite{altCntry,demonymCntry}, then refined by hand to ensure completeness with repect to potential forms, e.g. United States vs. The United States. For fun we added intialisms.
\item \textit{Rgn} is from the NGA GEOnet Names Server (GNS)~\cite{geoNet}. We filter for full name and BGN-approved local official name. We restrict our results to A, P,and L feature categories.
\item \textit{Natl} is sourced from wikipedia lists of demonyms~\cite{demonymCntry,demonymList}.
\end{enumerate}

\section{Leaked Information for 12 Point Fonts}\label{sec:12ptfonts-appdx}

\begin{table*}[h!]
    \caption{Leaked 12 point font information. 12 point font results for unadjusted and monospaced schemes are the same as Table~\ref{tab:nyt10}. Overall, 12 point font sizes leak slightly less information in dependent schemes than 10 point font sizes, however, the difference is not significant. For \emph{FILN} and \emph{FNLN} in Calibri, the larger font size leaked \emph{more} information, due to the displacement error created by space characters.}
    \label{tab:12ptfonts}
    \centering
    \begin{tabular}{l}
      \input{tab/nyt12}
    \end{tabular}
\end{table*}

We found that the leaked information for 12 point fonts is roughly equivalent
overall to that of a 10 point font: the amount of bits leaked is approximately
the same in all cases, showing that the information leaks scale across font sizes.
We report our results in Table~\ref{tab:12ptfonts}.

Note that we do not reproduce the independent scheme results for this table since they are identical to Table~\ref{tab:nyt10}.

\section{Redaction Location}\label{sec:redact-loc-appdx}

\begin{table}[h!]
  \centering
  \caption{Accuracy of locating nontrivial redactions using a box-walk routine vs. Timothy B. Lee's method, which records graphics state draw commands and looks for rectangles. Here we seperate redactions into ``easy'' and ``hard'' categories, where ``hard'' redactions are, for example, boxes drawn in the document with no surrounding text, or redactions that extend across and entire line and thus are too long to attack.}
  \label{tab:redactfind}
  \include{tab/redact-find}
\end{table}

In Table~\ref{tab:redactfind} we report the comparison between our algorithm for locating nontrivial redactions and the one provided by Timothy B. Lee~\cite{timblee}.
We give an outline of this algorithm in Figure~\ref{fig:nontriv-alg}.
This algorithm, we note, is optimized to find boxes with respect to \emph{other non-redacted words} on the page, whereas Lee's method looks for rectangle draw commands.
Lee's method is therefore better at detecting redactions with no surrounding text, but these redactions are less useful for the deredaction attacks on nontrivial redactions presented in this paper.
We also added a second step to the x-ray algorithm~\cite{xrayTool} for locating trivial redactions which removed a large number of false positives from the results (algorithm in Figure~\ref{fig:xray-alg}).

These bash scripts call into C, python, and ruby for various subroutines. 
The ``pts'' command is our own, and handles lifting a PDF specification into an intermediate representation consisting of glyph coordinates at the scale of displacment units, mentioned briefly in Section~\ref{sec:maxray}.
\url{find\_redaction\_box.py} and \url{trivial\_redaction\_loc.py} work as described earlier in this paper.
The former checks every sufficiently large space between two words for a redaction rectangle and the latter compares the pixels of the two rasterized images at glyph coordinates piped in by \url{get\_word\_coords.rb}.

\lstset{ %
language=bash,                % choose the language of the code
basicstyle=\ttfamily\footnotesize,       % the size of the fonts that are used for the code
numbers=none,                   % where to put the line-numbers
numberstyle=\ttfamily\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}

\begin{figure}[h!]
\begin{lstlisting}
tf=$(mktemp -u)
# Removes images from PDF
cpdf -draft "$1" -o "$tf".pdf-0
$SRC/painting/remove-tjs.sh "$tf".pdf-0 "$tf".pdf
convert -background 'rgb(255,255,255)' \
        -colorspace gray -normalize \
        -density 300 -quality 100 -depth 8 \
        "$tf".pdf "$tf".ppm 2>/dev/null
# parses out all the PDF text state and
# walks redaction boxes
$SRC/c-src/pts "$1" 1 |
    $SRC/location/find_redaction_box.py "$tf".ppm
\end{lstlisting}
\caption{Nontrivial redaction location algorithm}
\label{fig:nontriv-alg}
\end{figure}

\begin{figure}[h!]
\begin{lstlisting}
# convert all text to black
"$DIR"/lib/camlpdf -blacktext "$1" -o "$1"-a
# remove all text from one pdf
gs -q -o "$1"-b \
   -sDEVICE=pdfwrite -dFILTERTEXT "$1"-a
# create two ppms
pdftoppm -singlefile -r 300 "$1"-a "$1"-a
pdftoppm -singlefile -r 300 "$1"-b "$1"-b
# get coordinates of each word and compare pixels for differences
"$DIR"/get_word_coords.rb "$1"-a |
  "$DIR"/trivial_redaction_loc.py \
  "$1"-a.ppm "$1"-b.ppm
\end{lstlisting}
\caption{Two-pass algorithm for locating trivial redactions}
\label{fig:xray-alg}
\end{figure}

\section{PDF Workflows}

We peformed an analysis of several different PDF document production workflows across a variety of operating systems and software.
Our results are reported in Table~\ref{tab:pdfflows}.
This table demonstrates the wide variety of of schemes and transfer functions for displacements in different software sets.
Each row grouping represents a different general environment and software creator for the production of the PDF document, and each row represents a specific workflow---mostly which buttons are pressed during the PDF's creation.

\begin{table*}
  \centering
  \caption{Several different possible PDF workflows. Each entry in the column on the left should be read from left to right, indicating the stages used to produce the document. For example, ``Edge/Firefox, Print/PDFViewer, Save'' can be interpreted as ``using the edge or firefox browsers’ PDF viewer or print dialog, hit save'' and results in the right column's displacements.}
  \label{tab:pdfflows}
  \include{tab/flows}
\end{table*}

\section{The Acrobat Pro Displacement Scheme}
\label{sec:acro-pro-deets}

We can divide the effects of Acrobat Pro on PDF displacements along into two functionalities: document editing and document OCR.
Clicking on the text of an existing PDF in Acrobat does not change any positioning information.
However, when a user edits a text object (typically one line of text) Acrobat sets all the object's displacements to 0, making the scheme unadjusted.
During OCR, Acrobat (1) creates text objects and (2) adds noise to otherwise unadjusted text.
Acrobat's OCR algorithm creates displacement noise by adding character and word spacing operators to each word, starting at the first letter of each word.
The former, \texttt{Tc}, adds a small displacement to each character in the word.
The latter, \texttt{Td}, adjusts the word's x,y coordinates relative to the end of the prior word.
When redaction tools remove text metadata, the metadata may include these spacing operators.
Therefore, a redaction's width is not necessarily equivalent to the removed glyphs' cumulative advance width, posing an additional challenge for deredaction.
However, we found these operators' parameters leak via two sidechannels:

\begin{enumerate}
    \item \textbf{Tc}: This operator also applies to the successor space character of the word. 
        Since this space is rarely redacted, the applied Tc command remains in the PDF after redaction.
        We validated this for all redaction tools in Section~\ref{sec:tools}.
    \item \textbf{Td}: All of Section~\ref{sec:tools}'s redaction tools draw a box after removing metadata to indicate a redaction.
        This black or white box's coordinates match those of the first glyph in the redacted word \emph{after} the Td adjustment, revealing the redaction's exact width.
        If redaction removes the word's predecessor space character, this sidechannel is removed.
\end{enumerate}

As a result, if a document is run through Acrobat's OCR before redaction and these sidechannels are not removed.
Redactions of documents produced by Acrobat's OCR are therefore not much more secure than PDFs with an unadjusted displacement scheme.

% NOTE: include if we want to assume the space character is not there
% If the ``image conversion'' flow is used, the inferred inter-character spacing transform is smaller.
% To validate this empirically, we created 10 pages worth of 300 DPI pngs using the Edge browser, Word 365, the simple ``Save as PDF'' workflow, and ImageMagick's convert tool, in 10pt and 12pt sizes, for Times New Roman, Arial, and Calibri fonts from text sampled out of the NYT corpus used in Section~\ref{sec:eval}.
% For each space-separated string in this text we measured the inferred character spacing.
% We found the average character spacing value was XXX displacement units, with a median of XXX units, a maximum of XXX units, and a std. of XXX units.\footnote{Note \texttt{Tc} values set in the Adobe UI below 0.01 are rounded to 0, so we can use these units to infer the image converter (OCR) created a PDF.}
% Where the smaller variety of spacing is seen, this error is low enough that even without our ``space hack'' from the prior paragraph, documents using Adobe's OCR are vulnerable so long as redaction is applied after the OCR process and a one displacement unit error is taken into account.

\lstset{ %
language=C++,                % choose the language of the code
basicstyle=\ttfamily\footnotesize,       % the size of the fonts that are used for the code
numbers=none,                   % where to put the line-numbers
numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}


\begin{figure}
\begin{lstlisting}
int i = 0;
int trackingAdj = 0;
do {
  int accumulatedDiff = 0;
  int lastNewAdj = 0;
  int totalWidth = 0;
  int amountAdjustedSoFar = 0;
  totalWidth += fontScaledWidths[i];
  int newAdjustment = PIXEL_W(totalWidth);
  accumulatedDiff = pixelWidths[i] - newAdjustment;
  pixelWidths[i] = amountAdjustedSoFar = lastNewAdj = newAdjustment;
  uncorrectedPixelWidths[i] = newAdjustment;
  i++;
  if (i == numChars)
    break;
  do {
    totalWidth += fontScaledWidths[i];
    if (totalWidth > WIDTH_BRKPOINT)
      break;
    int origAdjustment = pixelWidths[i];
    int newAdj = PIXEL_W(totalWidth);
    newAdj -= amountAdjustedSoFar;
    int adjustmentDifference = origAdjustment - newAdj;
    trackingAdj = adjustmentDifference - accumulatedDiff;
    if (adjustmentDifference != accumulatedDiff) {
      int v28 = trackingAdj & 1;
      int v50 = trackingAdj & 1;
      if (trackingAdj <= 0) {
        trackingAdj >>= 1;
        if (adjustmentDifference < -accumulatedDiff)
          trackingAdj += v50;
        if (-newAdj >= trackingAdj)
          trackingAdj = -newAdj;
      } else {
        trackingAdj >>= 1;
        if (accumulatedDiff < -adjustmentDifference)
          trackingAdj += v28;
        if (lastNewAdj < trackingAdj)
          trackingAdj = lastNewAdj;
      }
    }
    pixelWidths[i - 1] -= trackingAdj;
    int newTrackAdj = newAdj + trackingAdj;
    amountAdjustedSoFar = amountAdjustedSoFar + newAdj;
    accumulatedDiff = origAdjustment - (newTrackAdj);
    pixelWidths[i] = newTrackAdj;
    uncorrectedPixelWidths[i] = newTrackAdj;
    lastNewAdj = newAdj;
    i++;
  } while (i < numChars);
} while (i < numChars);
\end{lstlisting}
\caption{Word WYSIWYG width adjustment method.}
\label{fig:wysiwyg-alg}
\end{figure}


\begin{figure}
\begin{lstlisting}
if (msword_year <= 2016) {
  int leadingSpace = 1;
  float dev = 0;
  float ttf = 0;
  for (int j = i + 1; j < vs->size(); j++) {

    if (vs->getChar(j) == ' ' && leadingSpace) {
      continue;
    } else if (leadingSpace) {
      leadingSpace = 0;
    }

    float t = textSpaceWidths2007[j] / 1000;
    double d = deviceWidths[j] / msFSize2007;

    ttf += t;
    dev += d;
    double disp = ttf - dev;
    if ((disp > 0.003 || disp < -0.003) && i != vs->size() - 1) {
      int adj = disp * 1000 + 0.5;
      vs->setDisplacement(j, adj);
      ttf = dev = 0;
    } else {
      vs->setDisplacement(j, 0);
    }
  }
} else {
  int leadingSpace = 1;
  float dev = 0;
  float ttf = 0;
  float t = 0;
  float d = 0;
  double disp = 0;
  for (int j = i + 1; j < vs->size(); j++) {

    if (vs->getChar(j) == ' ' && leadingSpace) {
      continue;
    } else if (leadingSpace) {
      leadingSpace = 0;
    }

    t = textSpaceWidths2019[j] / 1000;
    d = deviceWidths[j] / msFSize2019;

    ttf += t;
    dev += d;
    disp = ttf - dev;

    if (((disp > 0.003) || (disp < -0.003)) && i != vs->size() - 1) {
      int adj = disp * 1000 + 0.5;
      vs->setDisplacement(j, adj);
      ttf = dev = 0;
    } else {
      vs->setDisplacement(j, 0);
    }
  }
}
\end{lstlisting}
\caption{Adjustment routine for Word's displacment scheme}
\label{fig:adjust-alg}
\end{figure}

\begin{figure}
\begin{lstlisting}
   std::vector<double> Office::computeEditAdjustments(VectorString *vs) {
       std::vector<double> editAdjustments;
       int totalDots = 0;
       double totalDevWidth = 0;
       for (int i = 0; i < numChars; i++) {
           totalDots += (i == numChars - 1) ? uncorrectedPixelWidths[i] : pixelWidths[i];
           totalDevWidth += (textSpaceWidths2019[i] - vs->getDisplacement(i)) * (msFSize2019 / 1000);
           double realWidth, editedWidth, adj;
           realWidth = totalDevWidth + dotsToPdfUnits2019(600);
           editedWidth = roundToDigits(dotsToPdfUnits2019(totalDots + 600), 5);
           adj = (realWidth - editedWidth) / (msFSize2019 / 1000);
           editAdjustments.push_back(adj);
       }
       return editAdjustments;
   }
   std::vector<double> Office::edit(VectorString *vs, std::vector<double> eAdjs, int i) {
       double disp;
       disp = roundf(eAdjs[i] * (msFSize2019 / 1000) * 1000) / 1000 / (msFSize2019 / 1000);
       vs->addDisplacement(i, disp);
       adjust(vs, i);
       return computeEditAdjustments(vs);
   }
   void Office::editSuffix(std::vector<double> savedEAdjs, VectorString savedVs, VectorString *suf) {
       double guessDisp;
       double checkDisp;
       double adjDisp;
       bool matches = true;
       for (int i = 0;i < suf->size()-1;i++){
           int ind = savedVs.size() - suf->size() + i;
           guessDisp = roundf(10 * savedVs.getDisplacement(ind));
           checkDisp = roundf(10 * suf->getDisplacement(i));
           if (ind == savedVs.size() - 1) {
               savedVs.setDisplacement(ind, suf->getDisplacement(i));
               break;
           }
           adjDisp = roundf(10*savedEAdjs[ind]);
           if (guessDisp + adjDisp == checkDisp) {
               savedEAdjs = edit(&savedVs, savedEAdjs, ind);
           } }
       for (int i = 0;i < savedVs.size()-1;i++){
           if (savedVs.getChar(i) == L'-') {
               savedEAdjs = edit(&savedVs, savedEAdjs, i - 1);
               savedEAdjs = edit(&savedVs, savedEAdjs, i);
           } } }
\end{lstlisting}
\caption{Microsoft Word edit history positioning scheme algorithm.}
\label{fig:edit-alg}
\end{figure}


\begin{figure}
\begin{lstlisting}
for (int i = 0; i < numChars; i++) {
  fontScaledWidth = widths[i] * fontSize * 2;
  fontScaledWidths.push_back(fontScaledWidth);
  if (msword_year == 2007) {
    float textSpaceW =
        roundf(roundf(((float) widths[i]) / UNIT_TEXT_SPACE_2007 * 10000) / 10);
    textSpaceWidths2007.push_back(textSpaceW);
  } else {
    double textSpaceW = roundf(((double) widths[i]) / UNIT_TEXT_SPACE_2019 * 1000.0);
    textSpaceWidths2019.push_back(textSpaceW);
  }
  uncorrectedPixelWidths.push_back(0);
}
if (justif) {
  justify();
}
computeWYSIWYG();
\end{lstlisting}
\caption{Word initialization of widths.}
\label{fig:initalg}
\end{figure}

\subsection{Microsoft Word Displacement Scheme}
\label{sec:mic-word-deets}

While other displacement schemes leak proportional width information, any accumulation of information conditioned on redacted glyphs potentially leaks information.
One such case is the WYSIWYG behavior of Microsoft Word PDF writers dating back to 2007.
Appendix~\ref{sec:word-disp-appdx} discusses \maxray's positioning scheme models.

Additional redacted information leaks occur because Microsoft Word's \emph{Save As PDF} tool converts between two glyph coordinate representations.
When users edit or create a Word document, they operate on a virtual document representation, internal to Word.
This representation determines how Word displays the document in the graphical user interface (GUI).
Note, however, the resolution of the user's screen and other environmental factors do not effect this virtual representation.
Included in the virtual document's representation are a set of \emph{internal widths} used to represent glyphs' sizes.
When Word writes a PDF file, it converts this virtual representation into a PDF specification.
The PDF file contains a seperate glyph width mapping, typically matching the embedded TrueType font file.
For unnecessary reasons, a small amount of error exists between the two representations' rendering specifications.

A glyph's virtual width representation can be smaller or larger than that same glyph's PDF width specification.
To account for this error, Word's PDF document writer accumulates each glyph's width error from left to right across each line of text twice.
The first pass modifies the internal representation of each character's width according to the difference between the current internal width and the TTF width of the line's prefix up to the current position, at around a 600 DPI resolution.
In the second pass, a second left-to-right accumulation occurs, accounting for error between the widths output by the first pass ad the TTF line width, converted to displacement units (typicaly 1/1000th of the font size at 72 DPI).
When the accumulated error hits a three displacement unit threshold, Word writes a displacement to the PDF and resets the accumulator.
In summary, the font metrics of the line to the left of any given threshold value effect the accumulated error, leaking redacted information via the redaction's width and non-redacted glyph displacements.\footnote{
    Monospace fonts do not contain conversion width errors.
}
For example, a redacted glyph with a 10 displacement unit error will overflow the accumulator and the glyph's effective PDF width will be its original advance width plus a displacement between 7 and 13 units depending on the accumulator's state before overflow.

We note the line's specific character ordering affects the accumulator state as different orderings will lead to different accumulator overflow positions.
For example, the accumulated error could fluctuate between postive and negative three displacment units for several characters and then overflow.
Both the point of overflow and the magnitude are conditioned on prior glyphs' modification of the accumulated error value.
For example, in Times New Roman, the digits 0 through 9 have no error and do not contribute to the accumulator.
However \emph{a lack} of displacement can also leak information about the redacted content.
Additionally, due in part to the algorithm's first pass, smaller fonts leak more information as they have more characters per line and more threshold opportunities.

We validated \maxray's models for Word versions between 2007 and 2019 using several fonts on hundreds of lines of text from Wikipedia, hundreds of manual tests, and thousands of real-world cases in Section~\ref{sec:wild}.
Section~\ref{sec:wild} describes \maxray's process for correctly identifying Word positioning schemes.
We also note that Microsoft Word's positioning scheme metadata depends on the Word document's edit history.
Appendix Figure~\ref{fig:edit-alg} gives code for edit history modeling.
Not all divisions effect glyph positioning and deciding which glyph positions to apply edits to requires a combinatoric search, so the bulk evaluations of Sections~\ref{sec:eval} and~\ref{sec:wild} do not model edits.

\subsubsection{Word Displacement Algorithms}\label{sec:word-disp-appdx}

The first routine (Figure~\ref{fig:initalg}) intializes a set of widths from two files, widths corresponds to TTF widths, and pixelWs are Word's internal widths for each character. It then initializes the WYSIWYG sizes.
The next routine (Figure~\ref{fig:wysiwyg-alg}) handles calculating the WYSIWYG widths for each character by accumulating errors between the two width representations, consisting of a tested loop that checks sets of runs of characters:
Then (Figure~\ref{fig:adjust-alg}), once an actual line of text needs to be adjusted, the deviceWidths initialized during the WYSIWYG modification are checked for overflow. 
The types of floating point variables, e.g. float vs. double, are precisely chosen and must be identical to the original algorithm or the result will be incorrect.

\section{Latex, LibreOffice, Other PDF Producers}
\label{sec:other-prod}

\textbf{LibreOffice} LibreOffice~\cite{libreOffice} includes a PDF writer as part of its Visual Class Library (VCL), and, at the time of writing, embeds displacements in the drawHorizontalGlyphs method of the PDFWriterImpl class. 
This method appears to be similar to Microsoft Word in function: displacements are applied whenever the native advance width of the PDF glyph does not match the Pixel x,y coordinates that LibreOffice uses internally, derived from the SalLayout (layout engine) class.
However, LibreOffice does not use a second width map for the characters in a given font, and therefore likely leaks less redacted information than Microsoft Office's positioning scheme.

\textbf{\LaTeX\ (TeX Live)}
The determination of displacements inside \LaTeX\ is dependent upon the particular flow that is used~\cite{latexSource}.
For the pdfTeX flow, interglyph displacements are decided by the pdf\_begin\_string procedure. 
The \LaTeX\ glyph placement algorithm is quite complex, however, our analysis did find one section of the code for determining displacments appears to round the difference between the current horizontal glyph render position and the start of the current text object.
Depending on the precision of the rounding, this could leak additional information about the order of glyphs used.
Other flows, such as XeLaTeX, can optionally include more complex calculations that determine how to shrink and expand glyphs to fit a certain amount of space and may leak large amounts of redacted information.
However, \LaTeX\ redactions are uncommon.

\textbf{Other Producers}
We found other producers, such as iText, where the default is unadjusted text objects, are accounted for by the schemes presented in the main body of this paper (Section~\ref{sec:pdftext}).

\subsection{Document Scanners}
\label{sec:doc-scanners}
Many document scanners also come with OCR features.
We examined the output of three different document scanners: a Canon MP Navigator EX, Xerox AltaLink C8145, and HP MFP M227fdn.
Of the three, the Canon and Xerox machines provided built-in software for document OCR.
We examined the Canon's positioning scheme first, and found redactions on PDFs produced by this workflow to be equally as vulnerable to deredaction as unadjusted schemes.
The Xerox machine was not as simple: the Xerox machine's OCR text objects are positioned stochastically without space characters in between them.
After testing several redaction tools on the Xerox document, we found it was as vulnerable as a document with an unadjusted scheme as long as redaction was performed by removing glyphs rather than entire text objects.


==> cases-safe.tex <==
\section{Redacted Case Studies}
\label{sec:cases}
\label{sec:epstein}
\label{sec:snowden}
\label{sec:manafort}

We found deredaction is effective in \emph{targeted attacks}, where the size of the guess dictionary can be restricted by prior information.
Naively, we felt that the decision to perform this evaluation was justified insofar as we only deredacted powerful organizations, countries, and politicians.

We later found that the inclusion of the results in this section made readers and reviewers uncomfortable.
Though of less impact than the publication of nuclear chain reactions by Curie~\cite{}, the ethical concerns regarding the use of our findings are similar.

We therefore do not include any targeted deredaction results in the present version of this paper.
We validated our results extensively and are confident our findings are correct.
For each of the case studies, the individual using \maxray\ had no prior information besides the PDF pages studied.

Discussions with affected parties have led us to determine none of our evaluations will cause harm to individuals.
However, these techniques \emph{are} dangerous.
We discuss the matter of ethics futher in Section~\ref{sec:ethics}.


==> cases.tex <==
\section{Case Studies}
\label{sec:cases}

In this section we discuss targeted rather than comprehensive deredaction.
For each case study, the individual using \maxray\ had no prior information besides the PDF pages studied.

\subsection{United States v. Ghislaine Maxwell}\label{sec:epstein}
 
% https://www.nhpr.org/post/ghislaine-maxwell-accused-providing-girls-jeffrey-epstein-arrested-nh/
Ghislaine Maxwell was charged with crimes of enticement of minors and sex trafficking of underage girls~\cite{ghislaineMaxwell}.
% 1:20-cr-00330-AJN
As of the 28th of April 2021, Maxwell has been undergoing trial in The Southern District Court of New York~\cite{maxwellTrialDocket}.

We applied \maxray\ to several documents from this case.
Our location algorithms discovered \numEpsteinPagesRedacted\ pages matching Microsoft Word positioning schemes across \numEpsteinDocuments\ documents and located \numEpsteinRedactions\ redactions.
We did not attempt deredaction on occurrences where the redaction was too long or we could not reasonably determine a dictionary, resulting in \numEpsteinVulnRedactions\ vulnerable redactions.
\textbf{We also did not attempt to deredact any full names in the Maxwell documents, e.g. of witnesses, and none appear to be vulnerable to the discovered attacks.}

\begin{table*}
\centering
\caption{Redactions from \emph{real documents} attacked in this section. The ability to reveal this information poses a security risk.}
\begin{tabular}{ccc}
\toprule
Image & Document, Page & Deredacted Content \\
\midrule
{
        \begin{tabular}{c}
\includegraphics[width=3.5in]{fig/epstein-134-13.pdf} \\
        \end{tabular}
} & 
{
        \begin{tabular}{c}
Epstein 134, Page 13  \\
        \end{tabular}
} & 
{
        \begin{tabular}{c}
        the CIA \\
        \end{tabular}
} \\
\midrule
{
        \begin{tabular}{c}
\includegraphics[width=3.5in]{fig/libya.pdf} \\
        \end{tabular}
} & 
{
        \begin{tabular}{c}
Snowden, Page 10 \\
        \end{tabular}
} & 
{
        \begin{tabular}{c}
        Libyan, Libyan \\
        \end{tabular}
} \\
\midrule
{
        \begin{tabular}{c}
\includegraphics[width=3.5in]{fig/manafort.pdf} \\
        \end{tabular}
} & 
{
        \begin{tabular}{c}
Manafort, Page 64 \\
        \end{tabular}
} & 
{
        \begin{tabular}{c}
        Prodi \\
        \end{tabular}
} \\
\bottomrule
\end{tabular}
\end{table*}

\emph{Document 134, page 13.}
On page 13 of Document 134, a redaction indicates who ``had come to the government ... asking it to open an investigation ... [of] Epstein and Maxwell''.
% https://www.sec.gov/rules/other/4-460list.htm
We attempted deredaction using following dictionaries: all first name and surname pairs, first names, surnames with and without title, single and double word combinations (with and without the first letter capitalized), companies listed by the US Securities and Exchange Commission~\cite{secCompanies}, and five-letter acronyms.
We had \emph{no matches} for the given displacements.
We then tried three letter acronyms with a premodifier of ``the'', e.g. ``the FBI''.
This resulted in matches for 33 acronyms: the first letter was B, C or R, the second letter could only be I, and the third letter was one of 11 possibilities.
\emph{None} of these acronyms matched a known organization except one: the CIA.

Prior peer review found this result extraordinary, so we provide the following consolations:
\begin{itemize}
    \item ``had come to the government'' implies that the redacted content is not part of the government.
As the CIA is not typically involved in domestic affairs and does not serve the same role of the judicial branch, we do not feel this rules the CIA out as a possibility. The phrase may refer to the CIA as something other than ``the government'' because the agency is a service of the government.
    \item Whether the CIA were involved in identifying the case is of little importance and is not suprising or conspiratorial. 
          Providing law enforcement with information regarding Epstein is within the organization's purview and duty, especially considering this information may have been received through the agency's contact page for information regarding international affairs.~\cite{ciaTip}
    \item The CIA was the only result that matched given our dictionaries and we are of the opinion that our dictionaries are sufficient to remove reasonable doubt.
          However, we remain open to the possibility that the redacted content may be different: perhaps the original name has a typo or does not occur in the US Census or Social Security Administration first name database.
          The nature of redaction does not \emph{absolutely guarantee} that this is the final redacted content. 
\end{itemize}

Another three redactions were deredacted to 114, 367, and 105 possible original texts.
The results are as follows:

1. % \censor{because she [Maxwell] reasonably believed $X$ was and} \\
%      \censor{would remain private under the Protective Order We  xxx}  \\
%      \censor{tried all pairs of two english words and of the hundred xx}  \\
%      \censor{results only ``her testimony'' made sense in the context xx} \\ 
      Only one redacted text was likely used given the context.

2. % \censor{The government did indeed have previous contact with} \\
%      \censor{We tried singular and paired english word} 
      Of four hundred results, only two made sense in context.

% her kids or liberals
3. % \censor{... what was said between the government and X. Based} \\
%      \censor{upon the context, this appears to be the witnesses' first x} \\
      % \censor{name.} 
        Not enough information exists in this document to deduce the 
      \censor{witnesses' full name}, though a reduction to 105 possibilities from 
      111,472 is significant.

% \emph{Unmatched case.}
% We were unable to find a match for \censor{the last of the five redactions}.
% This redaction's content is likely not in \maxray's dictionaries.
% We had 3,899 matches for width, reduced from a guess set size of 1,296,569. 
% No guess matched the given displacements so this document may use a marginally different workflow than Word's \emph{Save As PDF}.
% However, if we identified the correct scheme, \maxray\ ruled out over a million possible redacted texts.

\subsection{Top Secret Snowden-leaked Document}\label{sec:snowden}

In 2013, Edward Snowden leaked Top Secret documents to news organizations, revealing the NSA was spying on American citizens without their consent~\cite{snowdenRevel}.
One document details a co-travel technology used to track the movements of foreign diplomats across countries~\cite{topSecretDoc}.

Our location methods identified 9 named entity redactions matching Word positioning schemes, only one of which was too long to guess.
We report our results in italics below.
When multiple matches occurred we report them in italics.

% 1403
% 1428
1. The targeted handsets were observed ... between known $Libyan$\footnote{The line's displacements were not an exact match (Appendix~\ref{sec:snowden-diffs}), but Libyan matched the redaction's width. The second case matched line displacements and widths.} government and military installations ... handsets ... were inferred to be $Libyan$ government forces.
% 1406 - too long
% 1408 

2. ... filter in or out ... co-travelers with specified prefixes (for instance, return only $[Russian,Omanis]$ mobiles
% 1410 - no suffix
% \item analytic will not be effective for large queries across multiple countries and large time frames (e.g., anywhere in $[No suffix]$ over the past year
% 1415

3. ... target travel across spanning countries of interest (e.g., \emph{[No match, likely variation of some name in dictionary]})
% 1424 - no suffix
% \item Locations are defined by CELL IDs (for GSM) or GEO-Hashes (for $[no suffix]$ any other selectors with Lat/Long).
% 1429

4. ... (e.g., ignore activity in $Albania$ or use only ...
% 1432 - 1408 correctness dependent
% 1434

5. over the past year and then anywhere in \emph{Liberia [France or Eritrea when accounting for Word editing behavior.]}\footnote{
We briefly mentioned such cases in Section~\ref{sec:ms-word}.
}
% 1449 - no prefix/suffix
% 1456

6. ... was tested using an $Indonesian$ terrorist case study.
% 1471 - no suffix
% \item Currently, the system is integrated with RT-RG, operating on $XXX$ GSM data.

7. Project codename for the ``Meet \& Greet Spatial Chaining Analytic''.
Width and NSA naming conventions suggest the redacted codename is a four-to-five letter acronym.
CMap leakages reduce the space to 8,294,400 possible codenames: \maxray\ narrows this down to \emph{3,528 codenames}. 
Less than 20 results match English words.

We reached out to the journalists behind this document's release.
They confirmed the Washington Post redacted the document rather than Snowden or the NSA.
As the document has been widely distributed and multiple vulnerable versions of the PDF exist online, no reasonable mitigation exists for the discovered vulnerabilities.

\subsection{United States v. Paul J. Manafort, Jr.}\label{sec:manafort}

Paul Manafort's two criminal trials started due to investigation into Russian interference in the 2016 presidential election.
The first trial began in July of 2018, with Manafort facing 18 criminal counts.
We focus on a trip itinerary and emails surrounding a redacted Prime Minister's visit to the United States, exhibits G and H of\ \cite{manafortTrial}.\footnote{
    We discuss the displacement scheme of this document in Appendix~\ref{sec:manafort-scheme}.
}


\maxray\ located 79 redactions, though many were too wide to attack.
We deredacted congresspeople who met with the prime minister, the prime minister's name, and the embassy providing transportation.
We note that the researcher running \maxray\ did not read the document in question.
\emph{The results below were achieved ``blind'' with respect to the document's content.}

\emph{The Embassy.}
Pages 60 and 61 have two redactions indicating the embassy providing transportation.
Both matched \emph{Italian}.
The next closest result, Welsh, was five units away from the correct width in both cases.

\emph{The Prime Minister.}
Four redactions on pages 63 and 64 determine the Prime Minister / President.
% https://en.wikipedia.org/wiki/List_of_state_leaders_in_the_20th_century_(1951%E2%80%932000)
% https://en.wikipedia.org/wiki/List_of_state_leaders_in_the_21st_century
We used a dictionary of world leaders (surnames) starting from 1951 until present day, totaling 4,281 names.~\cite{listStateLeaders}
These four redactions occurred in three different fonts.
Different font metrics leak different information, so extraneous results were eliminated.
For two of the redactions \emph{(Romano) Prodi} was the only exact match, and the other two had four and three exact matches, respectively.
The only other match for all four redactions was (Wilhelm) Pieck, a German politician who died in 1960.

\emph{The meetings.}
Several redactions indicated members of the 113th congress Romano Prodi met with and the states they represented.
Our dictionaries were the 113th congress~\cite{113thcongress}, demonyms (Appdx.~\ref{sec:dictdetail}), and state acronyms.
We reproduce the attacked redactions below, redacted using the same methods as the source document.

\begin{enumerate}[nosep]
    \item Senator \censor{Chris Murphy}, D-\censor{CT}). 
% \item The \emph{Italian} Ambassador. We note that this was 2 displacement units away from an exact match due to the aforementioned fixed per-character displacement inference.
% \item \emph{}, Senior Policy Advisor
    \item Congressman \censor{Ed Royce} R-\censor{CA}).
    \item Congressman \censor{Bill Keating} (D-\censor{MA}).
    \item Congressman \censor{Dana Rohrabacher} R-\censor{CA}). % This redaction included the leading space character and destroyed the TJ break created by Acrobat's OCR (Appendix~\ref{sec:acro-pro-deets}); however, \censor{Dana Rohrabacher xxx} was the closest match by $\approx$30 units.
\end{enumerate}

% \paragraph{The Senator.}
% We do not include \maxray's reported guesses for the Senator on page 61 as this redaction had no information for crossvalidation.
% Unlike the above congress members, the senator's state was not separately redacted.
% This redaction also lost character-spacing information for the Senator's first name.
% Acrobat's OCR has this unlikely potential for information loss (Appendix~\ref{sec:acro-pro-deets}).

\paragraph{Validation.}
For this document, we were able to perform additional validation of our results.
We correlated guessed congresspeople with their guessed state acronyms and meeting location information---some pages indicated the meetings would be held in office buildings where the congresspeople worked at the time of the document's release.
For the prime minister, one of the other pages in the source document reveals that the redacted Prime Minister's name was, indeed, Romano Prodi.
We were not able to validate \maxray's guesses for the Senator on page 61.
Unlike the other congress members, this redaction had little contextual information.




==> disc-scrap.tex <==
\subsection{Unaddressed Information Losses}\label{sec:loss}

This paper did not address three important cases: attacking rasterized documents, typos and augmentation of redacted content, and unconstrained PDF edits using tools like inkscape.

\subsubsection{Rasterization}\label{sec:raster}

In this paper, we left the problem of document rasterization largely untouched due to the large number of documents suffering from metadata attacks alone.
Our original intention with this work was to attack black-box style raster redactions, but upon discovering the complexity of displacement schemes themselves, we found several preliminary works would be needed to properly explore \emph{how} images get generated from PDF documents.
We note that (typically, depending on the PDF document configuration), 72 displacement units correspond to one pixel in a 72 DPI image; this suggests the information loss occurring from rasterization may be too great to deredact text accurately, but for higher DPI, it may indeed still be possible.
It may also be possible to determine the accumulated affects of displacments in the anti-aliasing of pixels for certain PDF-to-image converters, and recover the Word displacements. 
We leave further exploration of this problem to future work.

\subsubsection{Typos, Changing Redacted Text}\label{sec:disc-editing}

Another source of ``information loss'' occurs when either the text underneath the redaction is changed to a meaningless value, such as ``X's'', and it is possible to check if any of these glyph-removal redaction styles have the same width as the redaction.
A potentially more difficult ambiguity to resolve is unintentional information loss due to typos; this will require further analysis and work to model typos in redacted text, and we leave this to future work.

\subsubsection{Unconstrained Edit Behaviors}\label{sec:editing-behavior}

To better understand how unconstrained editing of PDF documents affects deredaction we performed tests of Acrobat's editing behavior and found a variety of different transforms dependent upon the highlighted text selection and edit type.
Editing glyphs can trigger a split of the text-showing operator into two: this appears to be tied to the ``undo'' functionality.
Selecting just one character and adding inter-character spacing will create a displacement.
However, selecting multiple characters and performing the same operation will split the text showing operator use \texttt{Tc} for the left-exclusive and right-inclusive boundaries of the highlighted text selection, i.e. ``(,]''.
Inter-word spacing operators are also added when edits occur with respect to word boundaries.
Modeling these edits requires modeling the \emph{configurability} of the Adobe interface: inter-character spacing values (and thus displacements) can be entered as real numbers via the UI.
Theoretically, this is infinitely more complex than modeling edits to a Word document because the human operator can choose the input spacing, and the potential for false positives and bias in prediction is large.
None-the-less we have full confidence that with further human subjects tests, consideration of further information channels, and advanced modeling this problem can be made tractable.

\subsection{Dictionary Generation, NLP}\label{sec:disc-dict-gen}

The generation of effective dictionaries for use in attacking redactions is also something the current paper does not address.
We found that many redactions we attacked had \emph{no results} in Section~\ref{sec:nonsynth}; manual analysis of these cases makes us confident that this is due to incomplete dictionary modeling of potential name formats.
We seperate this problem into three relevant subproblems:

\begin{enumerate}
\item \textit{Semantic prediction.} Determining whether a redaction is a name, region, pronoun, etc. is currently a highly manual analysis: we attempted to use RoBERTa~\cite{liu2019roberta} to predict the part of speech and rank the resulting matches for our deredaction attacks, but found it to be insufficient to guarantee the accuracy we desired in evaluating our techniques. Future work will be needed on automatically determining the semantic content of redactions, so that cases of vulnerability may be more effectively analyzed.
  \item \textit{Dictionary content.} The dictionaries used to provide the evaluation of this paper we mostly in English and ASCII-text based. In developing this paper, we found a relative drought of high quality dictionaries to use in attacking redactions, and so had to develop our own from several sources (Appendix~\ref{sec:dictdetail}), but future work could provide, for example, a more robust and complete public dictionary of names and name variations across different languages and in unicode format.
  \item \textit{Text augmentations.} In the evaluation of Section~\ref{sec:nonsynth}, we included several titles such as ``Mr.'' along side our base dictionary of names, however, a much larger number of modifiers exists, such as the title ``Sgt.'' referring to a member of the military, or cases where slightly more or less than the name is redacted, e.g. a comma after the name is redacted along with the name. Enumerating and understanding the different possible modifications to redacted text is a complex subject and will require further work.
\end{enumerate}

==> eval-scrap.tex <==


XXX

\subsection{Results}
Table~\ref{tab:nyt10} provides results for four fonts, Courier, Times New Roman, Arial, and Calibri, in 10 point size.
While columns are subdivided into three positioning schemes, they describe two classes of information leak.
NA presents the unadjusted leaks from Sections~\ref{sec:gdocs} and~\ref{sec:adobe-ocr}.
W07 and W21 present the leaky Microsoft Word 2007 and 2021 positioning schemes from Section~\ref{sec:ms-word}.
These two columns indicate the information leaks have existed for more than a decade.

The left half of the table reports the mutual (leaked) information for each dictionary.
For example, $15.94 \approx 16$ bits are necessary to encode all words in FN and a redaction of a word in FN in 10 point Calibri font and matching the Microsoft Word 2021 positioning scheme leaks 13.8 of these bits.
The table's right half gives the probability redacted content is uniquely determined using post-redaction information.
For these cases, deredaction finds a single matching dictionary entry.
The top half reports uniform prior information dictionary distribution results.
The bottom half reports weighted distribution results.
Some dictionaries have a higher probability for a unique deredaction because the sets of words with matching positioning information are independent of the frequency distribution and a this distribution eliminates some possible redacted texts.


Courier is an exception to Table~\ref{tab:nyt10}'s results.
Monospaced fonts behave identically in Unadjusted and Microsoft Word positioning schemes. 
The residual width information in Courier after redaction leaks only the number of characters in the redacted word. 
The Courier column in Table~\ref{tab:nyt10} is equivalent to the entropy of the distribution of word lengths.
A redacted American surname in 10 point Courier font in a PDF created by Google Docs will leak \hyunytlnnadjrx\ bits of information.
If the redaction's font were Times New Roman, it would leak 2.8 times as much information.
If Microsoft Word 2021 created this PDF, changing the font to Times New Roman would leak 4 times as much information.
Calibri, the default font in Microsoft Office since 2007, leaks the most redacted information due to a greater variety of glyph widths than the other three fonts.

\emph{Experimental Limitations}
Table~\ref{tab:nyt10} has no results for the \emph{Str} dictionary under the uniform distribution using Word positioning schemes: simulating redaction of all \neltstr\ strings is prohibitively expensive. 
We obtained results for the unadjusted scheme by exploiting the structure of the dictionary.
We also do not consider longer redactions because of the computational overhead. 
We do not consider the distribution of PDF producers: this information can be redacted from the PDF file~\cite{australiaRedact} so we do not assume this knowledge and examine glyph positioning information in isolation.

In summary, we find that redacting a fragment of text from a PDF using common redaction tools does not necessarily redact the text, even if redacted glyph information is removed from the document.


==> intro-scrap.tex <==
For monospace fonts, such as Courier, a redacted word's width tells us the how many letters are in the word. (This is enough  to distinguish between the pronouns ``he'' and ``she,'' for example.)
Proportional fonts such as Times New Roman, whose glyphs do not all have the same width, disclose more information.
In one case, this was thought to be enough to infer the name of a country redacted from a classified document~\cite{egyptian}. 
However, this document contained a raster image of the text rather than text objects, limiting the precision of recovered width information.
We estimate a document rasterized to 300 Dots-Per-Inch (DPI) can leak about 8 bits of information about a redacted name (Section~\ref{sec:defenses}).

In an all-digital workflow, however, where a PDF is generated directly by a typesetting system, word processor, or ``Print to PDF'' print driver, there is no loss of precision due to rasterization: exact recovery of specified glyph positions and widths is possible.
Worse yet, documents originating from Microsoft Word leak information beyond the redacted text's width. 
We find redacting a name from a PDF produced by Microsoft Word can leak about 13 bits of redacted information, enough to uniquely determine the name in 3\% of cases.


%%%



In this work, we present a comprehensive investigation of PDF text redaction. 
First, we report on the information preserved by popular digital PDF redaction tools. We found that 
We find, alongside broken tools which preserve redacted text, all current non-rasterizing PDF redaction software retains the glyph positioning information necessary for the deredaction of short text fragments, such as personal names.

Next, we measure the redacted information leaked by different PDF document creation workflows.
We examine how a PDF's creator affects the glyph positioning information needed for deredaction. 
As noted, documents originating from Microsoft Word leak information beyond the redaction's width. 
Even scanned documents post-processed by OCR before redaction leak redacted texts' width.

To demonstrate this attack, we built a tool, called \maxray, to deredact fragments of

==> pdftext-scrap.tex <==


XXX

It should be noted that many document scanning workflows do also produce an Optical Character Recognition (OCR) overlay that consists of text objects. \notefor{Max}{Make ``text objects'' in previous sentence raster text with OCR overlay.} These OCR text objects are not rendered, but do allow the underlying text to be searched and copied. We can recover the width of the redacted text from such document and carry out the attacks described later in this paper.
\end{comment}

Adobe has \emph{two} workflows for OCR.
The first, called \emph{image conversion}, occurs when a raster document is opened in the \emph{edit} tab directly, causing Acrobat to generate a custom font matching the raster as closely as possible.

\noteby{KL}{Stopped here.}

Non-raster documents undergo this transform (but not the custom font generation) when a user edits a text object---clicking on the text will not destroy the original metadata.
The other OCR flow is present on the ``OCR'' tab.
This will not cause custom font generation and adobe will attempt to match an existing system font to the raster.
If the ``edit'' tab is clicked after the ``OCR'' tab (but OCR is not run) then the ``image conversion'' workflow is used instead.

Both of these flows added no displacements but added \texttt{Tc} (inter-character spacing) and \texttt{Td} (adjust x,y based on start of previous text-showing operator) graphics state operators (Section~\ref{sec:pdftext}).
We found differences in \texttt{Tc} and \texttt{Td} occur at a per-OCR-inferred word granularity, broken at the first letter of each word and including the suffix space character.
Redaction tools can remove this graphics state operator information from redacted text (Section~\ref{sec:tools}).
Of particular importance is the redaction of the \texttt{Td} operator deciding the start of each word.
Reverse engineering revealed complex OCR models (dependent upon the positioning of PNG text) determine this operator's value.
Despite this roadblocks, we were still able to attack the redact-after-OCR approach with complete confidence.
The parameters to the two operators could be revealed via two additional routes of information leakage:

\begin{itemize}
  \item Adobe adds the character spacing operator from the first character of the word to the successor space character and redaction will often preserve this successor space.
  \item During redaction, the left side of the box is not applied to the end position of the prior text-showing operator but the starting position of the redacted text showing operator, that is, the $x$ value \emph{after} the \texttt{Td} operator is applied.
\end{itemize}

Thus in a significant number of cases, such as the Mueller Report (Section~\ref{sec:cases}), documents processed by OCR before redaction just as vulnerable as documents that underwent no rasterization.

% NOTE: include if we want to assume the space character is not there
% If the ``image conversion'' flow is used, the inferred inter-character spacing transform is smaller.
% To validate this empirically, we created 10 pages worth of 300 DPI pngs using the Edge browser, Word 365, the simple ``Save as PDF'' workflow, and ImageMagick's convert tool, in 10pt and 12pt sizes, for Times New Roman, Arial, and Calibri fonts from text sampled out of the NYT corpus used in Section~\ref{sec:eval}.
% For each space-separated string in this text we measured the inferred character spacing.
% We found the average character spacing value was XXX displacement units, with a median of XXX units, a maximum of XXX units, and a std. of XXX units.\footnote{Note \texttt{Tc} values set in the Adobe UI below 0.01 are rounded to 0, so we can use these units to infer the image converter (OCR) created a PDF.}
% Where the smaller variety of spacing is seen, this error is low enough that even without our ``space hack'' from the prior paragraph, documents using Adobe's OCR are vulnerable so long as redaction is applied after the OCR process and a one displacement unit error is taken into account.

%%%%

% %PDF is a text-based file format that describes how a document should appear, whether on screen or on paper, in an application-neutral way. PDF documents can contain both raster images and vector graphics specified using drawing operators.


\begin{comment}
\emph{PDF Writers} use a combination of these adjustments and other graphics state operators to format a PDF's text (Section~\ref{sec:flows}).
Glyphs are represented using Character IDs (CIDs) given by the (potentially incomplete) \emph{character map} of a corresponding font dictionary object.
This object is also responsible for describing the glyph widths and vector graphics (usually by referencing an embedded TTF file, though these maps can be incomplete as well).
For example, the introduction of this paper is represented \texttt{[(Ef)25(fecti)25(v)15(e)-498(d...]TJ}\footnote{URIs and other metadata are \emph{annotations} to this operator (separate objects).} as \LaTeX's PDF Writer uses a identity mapping for non-unicode characters and substitutes displacements for spaces. \note{I think we can delete this para.}

In horizontal writing mode, each character and displacement of a text-showing operator updates the x coordinate of the graphics state (a cell in the text matrix \texttt{Tm}) according to the glyph's \emph{advance}.
This advance may not match the dictionary-defined width exactly as it is also determined by the graphics state, which includes horizontal scaling, inter-character spacing, and other transforms.
During redaction, the redacted glyphs are removed from their associated text-showing operators, and their advances are replaced by other operators to preserve the positioning of non-redacted glyphs.
In Section~\ref{sec:tools}, we find these replacement operators preserve the width of the redacted text exactly. \note{Delete para.?}
\end{comment}


%%%


We also rendered the word ``AAAVVV'' in order to determine the effects of kerning; we note in the table where the results are significant (only Apple Pages and Acrobat workflows actually applied displacement for based on the TTF \texttt{kern} table and word flows did not include \texttt{kern} information).
We find many workflows leak more information about redacted text than width alone.
Following this discovery, we discuss on how some of these workflows leak and how deredaction leverages this information.
We treat the problem of correctly inferring a scheme in Section~\ref{sec:schemeid}.



Table~\ref{tab:flows} contains our baseline results for the default PDF Creator workflows of several closed-source software stacks.
We do not include XeTeX, pdftex, and LibreOffice in the table because their PDF Creator implementations are open source or Adobe Acrobat's editor because glyph displacements are configurable in the UI (Section~\ref{sec:editing-behavior}).
We find that most workflows are composed of some combination of transforms applied to the PDF document: for example, when printing a PDF from Word 365, Safari's PDF Viewer displaces glyphs by a linear function of the prior character's TTF width.

Several transforms are dependent on the ``Print to PDF'' driver version used (Section~\ref{sec:pdf-drivers}).
Identification of all possible combinations of transforms will likely require automated methods (Section~\ref{sec:flow-disc}).
Regardless, for a given scheme reverse engineering and careful measurement can deduce an algorithmic model.

%%%

\begin{figure*}
\centering
\begin{minipage}{2in}
\begin{tabular}{rl}
569 & ijlt \\
682 & Ifr \\
797 & Js \\
909 & acez \\
1024 & bdghknopquvxy \\
1139 & FPS \\
1251 & ELTZ \\
1366 & BCR \\
1479 & ADGHKNOQUVXYw \\
1593 & m \\
1821 & M \\
1933 & W \\
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}{2in}
\begin{tabular}{rl}
455 & ijl \\
569 & Ift \\
682 & r \\
1024 & Jcksvxyz \\
1139 & Labdeghnopqu \\
1251 & FTZ \\
1366 & ABEKPSVXY \\
1479 & CDHNRUw \\
1593 & GOQ \\
1706 & Mm \\
1933 & W \\
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}{2in}
\begin{tabular}{rl}
470 & il \\
490 & j \\
516 & I \\
625 & f \\
653 & J \\
686 & t \\
714 & r \\
801 & s \\
809 & z \\
861 & L \\
866 & c \\
887 & x \\
925 & v \\
927 & y \\
931 & k \\
941 & FS \\
959 & Z \\
964 & g \\
981 & a \\
998 & TY \\
1000 & E \\
1019 & e \\
1058 & P \\
1063 & X \\
1064 & K \\
1076 & bdhnpqu \\
1080 & o \\
1092 & C \\
1112 & R \\
1114 & B \\
1162 & V \\
1185 & A \\
1260 & D \\
1276 & H \\
1292 & G \\
1314 & U \\
1322 & N \\
1356 & O \\
1378 & Q \\
1464 & w \\
1636 & m \\
1751 & M \\
1822 & W \\
\end{tabular}
\end{minipage}
\\
\caption{Times, Arial, Calibri letter equivalence classes.}
\label{tab:letters}
\end{figure*}


%%%

\subsection{Attack Implementation}\label{sec:impl}
           
The Microsoft Word displacement schemes reimplemented in C.
Routines for attacking Adobe OCR and examining PDF files for the evaluation of later sections were built using a series of modular, UNIX/Plan9-style scripts, operating on glyph displacement abstractions provided by a augmented version of the Poppler PDF (xpdf) library, used by Qt and a number of other core Linux applications. 
We found that \emph{no} existing libraries for PDF file parsing contained correct APIs for performing the attacks in this work, so we wrote them.
The system operates by coordinating scripts with GNU Parallel~\cite{} to populate two databases, a PSQL database for storing parsed PDF document content and redaction metadata, and a MongoDB database for storing unstructured data relating to specific cases of redaction.
All parts of the system are performant enough to be run on a consumer laptop computer.


==> tab/corpora.tex <==
\begin{tabular}{lrrr}
\toprule
\emph{Statistic} & \emph{Wiki} & \emph{Legal} & \emph{XXX} \\
\midrule
Documents & XXX & XXX & XXX \\
Total words & XXX & XXX & XXX \\
Unique words & XXX & XXX & XXX \\
Word entropy & XXX & XXX & XXX \\
\bottomrule
\end{tabular}

==> tab/hybrid-synth-res.tex <==
\begin{tabular}{l@{\hspace{-0.35cm}}r@{\hspace{0.15cm}}rrrrr}
  \toprule
  Name    & Widths                                    & Matches & Rank    & $p_{coll}$ & 5\% Size & z-score \\
  \midrule
Kerr      & 1                                         & 14      & 1       & 2.45e-04   & 210      & 3.09    \\
Kur       & 2                                         & 3       & 3       & 6.37e-06   & 8049     & -1.0    \\
Seas      & 2                                         & 9       & 6       & 1.40e-05   & 3667     & -0.59   \\
Dain      & 5                                         & 92      & 27      & 3.44e-04   & 148      & -0.19   \\
Ilyas     & 6                                         & 9       & 1       & 7.58e-06   & 6769     & 1.77    \\
Ron       & 8                                         & 61      & 18      & 4.25e-04   & 120      & -0.14   \\
Kent      & 9                                         & 41      & 1       & 1.47e-04   & 348      & 6.16    \\
June      & 12                                        & 45      & 5       & 1.47e-04   & 348      & 1.62    \\
January   & 15                                        & 32      & 5       & 2.44e-04   & 210      & 0.03    \\
Hoggard   & 18                                        & 24      & 5       & 9.73e-05   & 526      & 1.3     \\
Petelin   & 26                                        & 110     & 105     & 3.12e-04   & 165      & -0.27   \\
Leith     & 28                                        & 56      & 7       & 2.61e-04   & 196      & 0.32    \\
Mylan     & 41                                        & 76      & 45      & 6.63e-04   & 78       & -0.22   \\
Litvak    & 43                                        & 143     & 31      & 6.38e-04   & 81       & -0.15   \\
Mohammad  & 44                                        & 51      & 4       & 3.92e-04   & 130      & 0.35    \\
Denver    & 47                                        & 211     & 58      & 7.73e-04   & 66       & -0.16   \\
Bernard   & 49                                        & 117     & 2       & 9.65e-04   & 54       & 2.65    \\
Elena     & 52                                        & 146     & 50      & 1.23e-03   & 42       & -0.19   \\
Katherine & 63                                        & 68      & 41      & 5.75e-04   & 90       & -0.15   \\
Delaney   & 65                                        & 91      & 2       & 3.29e-04   & 156      & 6.11    \\
Prieto    & 93                                        & 254     & 5       & 1.07e-03   & 48       & 3.36    \\
Savage    & 113                                       & 210     & 2       & 1.23E-03   & 42       & 4.93    \\
Nugent    & 163                                       & 342     & 3       & 1.12e-03   & 45       & 5.7     \\
October   & 172                                       & 294     & 266     & 1.34e-03   & 39       & -0.27   \\
Florida   & 374                                       & 795     & 181     & 5.46e-03   & 9        & -0.08   \\
Columbia  & 935                                       & 1106    & 194     & 4.60e-03   & 12       & -0.06   \\
Hummel    & 1489                                      & 2013    & 26      & 1.04e-02   & 4        & 1.2     \\
  \midrule
Avg nadj. & \multicolumn{2}{c}{\hybridNadjAvgMatches} & 318.2   & 3.49e-2 & 142        & 1.88               \\
Med nadj. & \multicolumn{2}{c}{643}                   & 23      & 5.57e-3 & 9          & 0.51               \\
Min nadj. & \multicolumn{2}{c}{\hybridNadjMinMatches} & 1       & 5.13e-5 & 3          & -0.32              \\
Max nadj. & \multicolumn{2}{c}{32,275}                & 2,568   & 0.19    & 1,000      & 10.8               \\
\bottomrule
\end{tabular}


==> tab/leakbits.tex <==
\begin{tabularx}{0.75\textwidth}{ll*{3}{*{5}{>{\raggedleft\arraybackslash}X}}}
\toprule
& & \multicolumn{4}{c}{\emph{Unadjusted}} & \multicolumn{3}{c}{\emph{Word 2016}} & \multicolumn{3}{c}{\emph{Word 2021}} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
\multicolumn{2}{l}{\emph{\textbf{Text}, Dict.}} &
\emph{Times} & \emph{Calibri} & \emph{Arial} & \emph{Mono}
& \emph{Times} & \emph{Calibri} & \emph{Arial}
& \emph{Times} & \emph{Calibri} & \emph{Arial} \\
\midrule
\multicolumn{2}{l}{\emph{\textbf{Uniform}}}
\\
& \emph{Str}
%& \hwxunistrt & \hwxunistrb & \hwxunistra & \hwxunistrm
%& \hwstrwxvit & \hwstrwxvic & \hwstrwxvia
%& \hwstrwxxit & \hwstrwxxic & \hwstrwxxia
\\
& \emph{Acrn}
%& \hwacrnpropt & \hwacrnpropc & \hwacrnpropa & \hwacrnpropm
%& \hwacrnwxvit & \hwacrnwxvic & \hwacrnwxvia
%& \hwacrnwxxit & \hwacrnwxxic & \hwacrnwxxia
\\
& \emph{Pron} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{Word} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{FN} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{LN} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{FILN} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{FNLN} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{Ctry} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{Rgn} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
& \emph{Natl} & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX & XXX \\
\bottomrule
\end{tabularx}

==> tab/nadjbits.tex <==
% DO NOT EDIT; this file is auto-generated by nadjbits.py

\begin{tabularx}{0.95\columnwidth}{ll*{4}{>{\raggedleft\arraybackslash}X}}
\toprule
\multicolumn{2}{l}{\emph{\textbf{Distr.,} Dict.}} &
\emph{Courier} & \emph{Times} & \emph{Arial} & \emph{Calibri} \\
\midrule
\multicolumn{2}{l}{\emph{\textbf{Uniform}}} \\
& \emph{Str} & \hyunytstrnadjrx & \hyunytstrnadjtx & \hyunytstrnadjax & \hyunytstrnadjbx \\
& \emph{Acrn} & \hyunytacrnnadjrx & \hyunytacrnnadjtx & \hyunytacrnnadjax & \hyunytacrnnadjbx \\
& \emph{Pron} & \hyunytpronnadjrx & \hyunytpronnadjtx & \hyunytpronnadjax & \hyunytpronnadjbx \\
& \emph{Word} & \hyunytwordnadjrx & \hyunytwordnadjtx & \hyunytwordnadjax & \hyunytwordnadjbx \\
& \emph{FN} & \hyunytfnnadjrx & \hyunytfnnadjtx & \hyunytfnnadjax & \hyunytfnnadjbx \\
& \emph{LN} & \hyunytlnnadjrx & \hyunytlnnadjtx & \hyunytlnnadjax & \hyunytlnnadjbx \\
\multicolumn{2}{l}{\emph{\textbf{News}}} \\
& \emph{Str} & \hywnytstrnadjrx & \hywnytstrnadjtx & \hywnytstrnadjax & \hywnytstrnadjbx \\
& \emph{Acrn} & \hywnytacrnnadjrx & \hywnytacrnnadjtx & \hywnytacrnnadjax & \hywnytacrnnadjbx \\
& \emph{Pron} & \hywnytpronnadjrx & \hywnytpronnadjtx & \hywnytpronnadjax & \hywnytpronnadjbx \\
& \emph{Word} & \hywnytwordnadjrx & \hywnytwordnadjtx & \hywnytwordnadjax & \hywnytwordnadjbx \\
& \emph{FN} & \hywnytfnnadjrx & \hywnytfnnadjtx & \hywnytfnnadjax & \hywnytfnnadjbx \\
& \emph{LN} & \hywnytlnnadjrx & \hywnytlnnadjtx & \hywnytlnnadjax & \hywnytlnnadjbx \\
\bottomrule
\end{tabularx}


==> tab/nyt10-static-eval.tex <==
\newcommand\nytxunknown{\raisebox{1.25pt}{---}}
\begin{tabular}{l@{\hspace{0.785em}}l@{}r@{\hspace{3pt}}*{3}{@{\hspace{6pt}}*{3}{@{\hspace{1pt}}r@{\hspace{1pt}}}}@{\hspace{12pt}}*{3}{@{\hspace{6pt}}*{3}{@{\hspace{1pt}}r@{\hspace{2pt}}}}}
\toprule
& &
& \multicolumn{9}{c}{Leaked information (bits)}
& \multicolumn{9}{c}{Probability correct guess} \\
\cmidrule(lr){5-11}\cmidrule(lr){14-20}
\multicolumn{2}{l}{\emph{\textbf{Distr}}} & {Courier}\kern-8pt
& \multicolumn{3}{c}{{\tfontname}\hspace*{10pt}}
& \multicolumn{3}{c}{{\kern-6pt\afontname}}
& \multicolumn{3}{c}{{\kern-16pt\bfontname}}
& \multicolumn{3}{c}{{\tfontname}}
& \multicolumn{3}{c}{{\afontname}}
& \multicolumn{3}{c}{{\bfontname}}
\\
& \emph{Dict}
& Mo
& {\nadjshortname} & {\wxiishortname} & {\wxxishortname}
& {\nadjshortname} & {\wxiishortname} & {\wxxishortname}
& {\nadjshortname} & {\wxiishortname} & {\wxxishortname}
& {\nadjshortname} & {\wxiishortname} & {\wxxishortname}
& {\nadjshortname} & {\wxiishortname} & {\wxxishortname}
& {\nadjshortname} & {\wxiishortname} & {\wxxishortname}
\\
\midrule
\multicolumn{6}{l}{\emph{\textbf{\uniname}}}
\\
& \emph{\strname}
& \hyunytstrnadjrx
& \hyunytstrnadjtx & \nytxunknown & \nytxunknown
& \hyunytstrnadjax & \nytxunknown & \nytxunknown
& \hyunytstrnadjbx & \nytxunknown & \nytxunknown
&	\textless1\%	&	\nytxunknown	&	\nytxunknown
&	\textless1\%	&	\nytxunknown	&	\nytxunknown
&	\textless1\%	&	\nytxunknown	&	\nytxunknown
\\
& \emph{\acrnname}
& \hyunytacrnnadjrx
& \hyunytacrnnadjtx & \hyuavgnytacrnwxiitx & \hyuavgnytacrnwxxitx
& \hyunytacrnnadjax & \hyuavgnytacrnwxiiax & \hyuavgnytacrnwxxiax
& \hyunytacrnnadjbx & \hyuavgnytacrnwxiibx & \hyuavgnytacrnwxxibx
% & \pgupctnytacrnnadjtx & \pguavgpctnytacrnwxiitx & \pguavgpctnytacrnwxxitx
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pgupctnytacrnnadjax & \pguavgpctnytacrnwxiiax & \pguavgpctnytacrnwxxiax
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pgupctnytacrnnadjbx & \pguavgpctnytacrnwxiibx & \pguavgpctnytacrnwxxibx
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
\\
& \emph{\wordname}
& \hyunytwordnadjrx
& \hyunytwordnadjtx & \hyuavgnytwordwxiitx & \hyuavgnytwordwxxitx
& \hyunytwordnadjax & \hyuavgnytwordwxiiax & \hyuavgnytwordwxxiax
& \hyunytwordnadjbx & \hyuavgnytwordwxiibx & \hyuavgnytwordwxxibx
% & \pgupctnytwordnadjtx & \pguavgpctnytwordwxiitx & \pguavgpctnytwordwxxitx
&	\textless1\%	&	10.2\%	&	8.2\% %pg
% & \pgupctnytwordnadjax & \pguavgpctnytwordwxiiax & \pguavgpctnytwordwxxiax
&	\textless1\%	&	9.5\%	&	5.8\% %pg
% & \pgupctnytwordnadjbx & \pguavgpctnytwordwxiibx & \pguavgpctnytwordwxxibx
&	11.7\%	&	33.0\%	&	33.0\% %pg
\\
& \emph{\fnname}
& \hyunytfnnadjrx
& \hyunytfnnadjtx & \hyuavgnytfnwxiitx & \hyuavgnytfnwxxitx
& \hyunytfnnadjax & \hyuavgnytfnwxiiax & \hyuavgnytfnwxxiax
& \hyunytfnnadjbx & \hyuavgnytfnwxiibx & \hyuavgnytfnwxxibx
% & \pgupctnytfnnadjtx & \pguavgpctnytfnwxiitx & \pguavgpctnytfnwxxitx
&	\textless1\%	&	3.1\%	&	2.2\% %pg
% & \pgupctnytfnnadjax & \pguavgpctnytfnwxiiax & \pguavgpctnytfnwxxiax
&	\textless1\%	&	2.1\%	&	1.4\% %pg
% & \pgupctnytfnnadjbx & \pguavgpctnytfnwxiibx & \pguavgpctnytfnwxxibx
&	5.1\%	&	17.7\%	&	14.4\% %pg
\\
& \emph{\lnname}
& \hyunytlnnadjrx
& \hyunytlnnadjtx & \hyuavgnytlnwxiitx & \hyuavgnytlnwxxitx
& \hyunytlnnadjax & \hyuavgnytlnwxiiax & \hyuavgnytlnwxxiax
& \hyunytlnnadjbx & \hyuavgnytlnwxiibx & \hyuavgnytlnwxxibx
% & \pgupctnytlnnadjtx & \pguavgpctnytlnwxiitx & \pguavgpctnytlnwxxitx
&	\textless1\%	&	3.6\%	&	2.2\% %pg
% & \pgupctnytlnnadjax & \pguavgpctnytlnwxiiax & \pguavgpctnytlnwxxiax
&	\textless1\%	&	3.1\%	&	1.8\% %pg
% & \pgupctnytlnnadjbx & \pguavgpctnytlnwxiibx & \pguavgpctnytlnwxxibx
&	4.4\%	&	18.9\%	&	16.5\% %pg
\\
& \emph{\filnname}
& \hyuavgnytfixlnnadjrx
& \hyuavgnytfixlnnadjtx & \hyuavgnytfixlnwxiitx & \hyuavgnytfixlnwxxitx
& \hyuavgnytfixlnnadjax & \hyuavgnytfixlnwxiiax & \hyuavgnytfixlnwxxiax
& \hyuavgnytfixlnnadjbx & \hyuavgnytfixlnwxiibx & \hyuavgnytfixlnwxxibx
% & \pguavgpctnytfixlnnadjtx & \pguavgpctnytfixlnwxiitx & \pguavgpctnytfixlnwxxitx
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pguavgpctnytfixlnnadjax & \pguavgpctnytfixlnwxiiax & \pguavgpctnytfixlnwxxiax
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pguavgpctnytfixlnnadjbx & \pguavgpctnytfixlnwxiibx & \pguavgpctnytfixlnwxxibx
&	\textless1\%	&	1.1\%	&	1.0\% %pg
\\
& \emph{\fnlnname}
& \hyuavgnytfnxlnnadjrx
& \hyuavgnytfnxlnnadjtx & \hyuavgnytfnxlnwxiitx & \hyuavgnytfnxlnwxxitx
& \hyuavgnytfnxlnnadjax & \hyuavgnytfnxlnwxiiax & \hyuavgnytfnxlnwxxiax
& \hyuavgnytfnxlnnadjbx & \hyuavgnytfnxlnwxiibx & \hyuavgnytfnxlnwxxibx
% & \pguavgpctnytfnxlnnadjtx & \pguavgpctnytfnxlnwxiitx & \pguavgpctnytfnxlnwxxitx
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pguavgpctnytfnxlnnadjax & \pguavgpctnytfnxlnwxiiax & \pguavgpctnytfnxlnwxxiax
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pguavgpctnytfnxlnnadjbx & \pguavgpctnytfnxlnwxiibx & \pguavgpctnytfnxlnwxxibx
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
\\
& \emph{\fsfnlnname}
& 3.8
& 9.9 & 14.7 & 14.3
& 10.2 & 14.8 & 13.9
& 14 & 16.7 & 16.5
% & - & - & - % pg
&	\textless1\%	&	1.5\%	&	1.1\% %pg
% & - & - & - % pg
&	\textless1\%	&	1.6\%	&	\textless1\% %pg
% & - & - & - % pg
&	\textless1\%	&	5.8\%	&	5.1\% %pg
\\
& \emph{\ctryname}
& \hyuavgnytctrynadjrx
& \hyuavgnytctrynadjtx & \hyuavgnytctrywxiitx & \hyuavgnytctrywxxitx
& \hyuavgnytctrynadjax & \hyuavgnytctrywxiiax & \hyuavgnytctrywxxiax
& \hyuavgnytctrynadjbx & \hyuavgnytctrywxiibx & \hyuavgnytctrywxxibx
% & \pguavgpctnytctrynadjtx & \pguavgpctnytctrywxiitx & \pguavgpctnytctrywxxitx
&	70.7\%	&	93.3\%	&	93.3\% %pg
% & \pguavgpctnytctrynadjax & \pguavgpctnytctrywxiiax & \pguavgpctnytctrywxxiax
&	70.7\%	&	87.1\%	&	87.1\% %pg
% & \pguavgpctnytctrynadjbx & \pguavgpctnytctrywxiibx & \pguavgpctnytctrywxxibx
&	\textgreater99\%	&	\textgreater99\%	&	\textgreater99\% %pg
\\
& \emph{\rgnname}
& \hyuavgnytrgnnadjrx
& \hyuavgnytrgnnadjtx & \hyuavgnytrgnwxiitx & \hyuavgnytrgnwxxitx
& \hyuavgnytrgnnadjax & \hyuavgnytrgnwxiiax & \hyuavgnytrgnwxxiax
& \hyuavgnytrgnnadjbx & \hyuavgnytrgnwxiibx & \hyuavgnytrgnwxxibx
% & \pguavgpctnytrgnnadjtx & \pguavgpctnytrgnwxiitx & \pguavgpctnytrgnwxxitx
&	\textless1\%	&	1.2\%	&	\textless1\% %pg
% & \pguavgpctnytrgnnadjax & \pguavgpctnytrgnwxiiax & \pguavgpctnytrgnwxxiax
&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
% & \pguavgpctnytrgnnadjbx & \pguavgpctnytrgnwxiibx & \pguavgpctnytrgnwxxibx
&	\textless1\%	&	4.1\%	&	3.8\% %pg
\\
& \emph{\natlname}
& \hyuavgnytnatlnadjrx
& \hyuavgnytnatlnadjtx & \hyuavgnytnatlwxiitx & \hyuavgnytnatlwxxitx
& \hyuavgnytnatlnadjax & \hyuavgnytnatlwxiiax & \hyuavgnytnatlwxxiax
& \hyuavgnytnatlnadjbx & \hyuavgnytnatlwxiibx & \hyuavgnytnatlwxxibx
% & \pguavgpctnytnatlnadjtx & \pguavgpctnytnatlwxiitx & \pguavgpctnytnatlwxxitx
&	57.4\%	&	87.1\%	&	87.1\% %pg
% & \pguavgpctnytnatlnadjax & \pguavgpctnytnatlwxiiax & \pguavgpctnytnatlwxxiax
&	50.0\%	&	87.1\%	&	81.2\% %pg
% & \pguavgpctnytnatlnadjbx & \pguavgpctnytnatlwxiibx & \pguavgpctnytnatlwxxibx
&	93.3\%	&	93.3\%	&	93.3\% %pg
\\
\multicolumn{6}{l}{\emph{\textbf{\empname}}}
\\
& \emph{\strname}
& \hywnytstrnadjrx
& \hywnytstrnadjtx & \nytxunknown  & \nytxunknown
& \hywnytstrnadjax & \nytxunknown  & \nytxunknown
& \hywnytstrnadjbx & \nytxunknown  & \nytxunknown
&	5.4\%	&	\nytxunknown	&	\nytxunknown
&	5.1\%	&	\nytxunknown	&	\nytxunknown
&	40.6\%	&	\nytxunknown	&	\nytxunknown
\\
& \emph{\acrnname}
& \hywnytacrnnadjrx
& \hywnytacrnnadjtx & \hywavgnytacrnwxiitx & \hywavgnytacrnwxxitx
& \hywnytacrnnadjax & \hywavgnytacrnwxiiax & \hywavgnytacrnwxxiax
& \hywnytacrnnadjbx & \hywavgnytacrnwxiibx & \hywavgnytacrnwxxibx
% & \pgwpctnytacrnnadjtx & \pgwavgpctnytacrnwxiitx & \pgwavgpctnytacrnwxxitx
&	8.8\%	&	40.6\%	&	20.3\% %pg
% & \pgwpctnytacrnnadjax & \pgwavgpctnytacrnwxiiax & \pgwavgpctnytacrnwxxiax
&	8.2\%	&	26.8\%	&	21.8\% %pg
% & \pgwpctnytacrnnadjbx & \pgwavgpctnytacrnwxiibx & \pgwavgpctnytacrnwxxibx
&	53.6\%	&	70.7\%	&	70.7\% %pg
\\
& \emph{\wordname}
& \hywnytwordnadjrx
& \hywnytwordnadjtx & \hywavgnytwordwxiitx & \hywavgnytwordwxxitx
& \hywnytwordnadjax & \hywavgnytwordwxiiax & \hywavgnytwordwxxiax
& \hywnytwordnadjbx & \hywavgnytwordwxiibx & \hywavgnytwordwxxibx
% & \pgwpctnytwordnadjtx & \pgwavgpctnytwordwxiitx & \pgwavgpctnytwordwxxitx
&	5.4\%	&	37.9\%	&	30.8\% %pg
% & \pgwpctnytwordnadjax & \pgwavgpctnytwordwxiiax & \pgwavgpctnytwordwxxiax
&	4.7\%	&	30.8\%	&	23.3\% %pg
% & \pgwpctnytwordnadjbx & \pgwavgpctnytwordwxiibx & \pgwavgpctnytwordwxxibx
&	46.7\%	&	70.7\%	&	66.0\% %pg
\\
& \emph{\fnname}
& \hywnytfnnadjrx
& \hywnytfnnadjtx & \hywavgnytfnwxiitx & \hywavgnytfnwxxitx
& \hywnytfnnadjax & \hywavgnytfnwxiiax & \hywavgnytfnwxxiax
& \hywnytfnnadjbx & \hywavgnytfnwxiibx & \hywavgnytfnwxxibx
% & \pgwpctnytfnnadjtx & \pgwavgpctnytfnwxiitx & \pgwavgpctnytfnwxxitx
&	15.4\%	&	57.4\%	&	46.7\% %pg
% & \pgwpctnytfnnadjax & \pgwavgpctnytfnwxiiax & \pgwavgpctnytfnwxxiax
&	16.5\%	&	46.7\%	&	40.6\% %pg
% & \pgwpctnytfnnadjbx & \pgwavgpctnytfnwxiibx & \pgwavgpctnytfnwxxibx
&	75.8\%	&	87.1\%	&	87.1\% %pg
\\
& \emph{\lnname}
& \hywnytlnnadjrx
& \hywnytlnnadjtx & \hywavgnytlnwxiitx & \hywavgnytlnwxxitx
& \hywnytlnnadjax & \hywavgnytlnwxiiax & \hywavgnytlnwxxiax
& \hywnytlnnadjbx & \hywavgnytlnwxiibx & \hywavgnytlnwxxibx
% & \pgwpctnytlnnadjtx & \pgwavgpctnytlnwxiitx & \pgwavgpctnytlnwxxitx
&	10.2\%	&	46.7\%	&	33.0\% %pg
% & \pgwpctnytlnnadjax & \pgwavgpctnytlnwxiiax & \pgwavgpctnytlnwxxiax
&	10.2\%	&	35.4\%	&	28.7\% %pg
% & \pgwpctnytlnnadjbx & \pgwavgpctnytlnwxiibx & \pgwavgpctnytlnwxxibx
&	57.4\%	&	81.2\%	&	75.8\% %pg
\\
& \emph{\filnname}
& \hywavgnytfilnnadjrx
& \hywavgnytfilnnadjtx & \hywavgnytfilnwxiitx & \hywavgnytfilnwxxitx
& \hywavgnytfilnnadjax & \hywavgnytfilnwxiiax & \hywavgnytfilnwxxiax
& \hywavgnytfilnnadjbx & \hywavgnytfilnwxiibx & \hywavgnytfilnwxxibx
% & \pgwavgpctnytfilnnadjtx & \pgwavgpctnytfilnwxiitx & \pgwavgpctnytfilnwxxitx
&	2.2\%	&	20.3\%	&	16.5\% %pg
% & \pgwavgpctnytfilnnadjax & \pgwavgpctnytfilnwxiiax & \pgwavgpctnytfilnwxxiax
&	1.8\%	&	15.4\%	&	10.2\% %pg
% & \pgwavgpctnytfilnnadjbx & \pgwavgpctnytfilnwxiibx & \pgwavgpctnytfilnwxxibx
&	17.7\%	&	43.5\%	&	40.6\% %pg
\\
& \emph{\fnlnname}
& \hywavgnytfnlnnadjrx
& \hywavgnytfnlnnadjtx & \hywavgnytfnlnwxiitx & \hywavgnytfnlnwxxitx
& \hywavgnytfnlnnadjax & \hywavgnytfnlnwxiiax & \hywavgnytfnlnwxxiax
& \hywavgnytfnlnnadjbx & \hywavgnytfnlnwxiibx & \hywavgnytfnlnwxxibx
% & \pgwavgpctnytfnlnnadjtx & \pgwavgpctnytfnlnwxiitx & \pgwavgpctnytfnlnwxxitx
&	\textless1\%	&	12.5\%	&	10.9\% %pg
% & \pgwavgpctnytfnlnnadjax & \pgwavgpctnytfnlnwxiiax & \pgwavgpctnytfnlnwxxiax
&	1.1\%	&	12.5\%	&	8.8\% %pg
% & \pgwavgpctnytfnlnnadjbx & \pgwavgpctnytfnlnwxiibx & \pgwavgpctnytfnlnwxxibx
&	8.8\%	&	30.8\%	&	28.7\% %pg
\\
& \emph{\fsfnlnname}
& 3.2
& 8.8 & 11.4 & 11.2
& 9 & 11.4 & 11
& 11.5 & 12.2 & 12.1
% & - & 1 & 1 % pg
&	7.2\%	&	43.5\%	&	37.9\% %pg
% & - & 1 & 1 % pg
&	8.2\%	&	43.5\%	&	33.0\% %pg
% & - & 1 & 1 % pg
&	46.7\%	&	75.8\%	&	70.7\% %pg
\\
& \emph{\ctryname}
& \hywavgnytctrynadjrx
& \hywavgnytctrynadjtx & \hywavgnytctrywxiitx & \hywavgnytctrywxxitx
& \hywavgnytctrynadjax & \hywavgnytctrywxiiax & \hywavgnytctrywxxiax
& \hywavgnytctrynadjbx & \hywavgnytctrywxiibx & \hywavgnytctrywxxibx
% & \pgwavgpctnytctrynadjtx & \pgwavgpctnytctrywxiitx & \pgwavgpctnytctrywxxitx
&	81.2\%	&	93.3\%	&	87.1\% %pg
% & \pgwavgpctnytctrynadjax & \pgwavgpctnytctrywxiiax & \pgwavgpctnytctrywxxiax
&	81.2\%	&	87.1\%	&	87.1\% %pg
% & \pgwavgpctnytctrynadjbx & \pgwavgpctnytctrywxiibx & \pgwavgpctnytctrywxxibx
&	93.3\%	&	93.3\%	&	93.3\% %pg
\\
& \emph{\rgnname}
& \hywavgnytrgnnadjrx
& \hywavgnytrgnnadjtx & \hywavgnytrgnwxiitx & \hywavgnytrgnwxxitx
& \hywavgnytrgnnadjax & \hywavgnytrgnwxiiax & \hywavgnytrgnwxxiax
& \hywavgnytrgnnadjbx & \hywavgnytrgnwxiibx & \hywavgnytrgnwxxibx
% & \pgwavgpctnytrgnnadjtx & \pgwavgpctnytrgnwxiitx & \pgwavgpctnytrgnwxxitx
&	10.9\%	&	40.6\%	&	30.8\% %pg
% & \pgwavgpctnytrgnnadjax & \pgwavgpctnytrgnwxiiax & \pgwavgpctnytrgnwxxiax
&	10.2\%	&	30.8\%	&	25.0\% %pg
% & \pgwavgpctnytrgnnadjbx & \pgwavgpctnytrgnwxiibx & \pgwavgpctnytrgnwxxibx
&	50.0\%	&	61.6\%	&	61.6\% %pg
\\
& \emph{\natlname}
& \hywavgnytnatlnadjrx
& \hywavgnytnatlnadjtx & \hywavgnytnatlwxiitx & \hywavgnytnatlwxxitx
& \hywavgnytnatlnadjax & \hywavgnytnatlwxiiax & \hywavgnytnatlwxxiax
& \hywavgnytnatlnadjbx & \hywavgnytnatlwxiibx & \hywavgnytnatlwxxibx
% & \pgwavgpctnytnatlnadjtx & \pgwavgpctnytnatlwxiitx & \pgwavgpctnytnatlwxxitx
&	87.1\%	&	\textgreater99\%	&	\textgreater99\% %pg
% & \pgwavgpctnytnatlnadjax & \pgwavgpctnytnatlwxiiax & \pgwavgpctnytnatlwxxiax
&	81.2\%	&	93.3\%	&	93.3\% %pg
% & \pgwavgpctnytnatlnadjbx & \pgwavgpctnytnatlwxiibx & \pgwavgpctnytnatlwxxibx
&	\textgreater99\%	&	\textgreater99\%	&	\textgreater99\% %pg
\\
\bottomrule
\end{tabular}


==> tab/nyt12-static-eval.tex <==
\newcommand\nytxunknown{\raisebox{1.25pt}{---}}
\begin{tabular}{lrr@{\hspace{3pt}}rr@{\hspace{3pt}}rr@{\hspace{3pt}}rr@{\hspace{3pt}}rr@{\hspace{3pt}}rr@{\hspace{3pt}}rr}
\toprule
& &
\multicolumn{6}{c}{Leaked information (bits)}
& \multicolumn{6}{c}{Probability unique match} \\
\cmidrule(lr){3-8}\cmidrule(lr){9-14}
\multicolumn{2}{l}{\emph{\textbf{Distr}}}
& \multicolumn{2}{c}{{\tfontname}}
& \multicolumn{2}{c}{{\afontname}}
& \multicolumn{2}{c}{{\bfontname}}
& \multicolumn{2}{c}{{\tfontname}}
& \multicolumn{2}{c}{{\afontname}}
& \multicolumn{2}{c}{{\bfontname}}
\\
&
\emph{Dict}
& {\wxiishortname} & {\wxxishortname}
& {\wxiishortname} & {\wxxishortname}
& {\wxiishortname} & {\wxxishortname}
& {\wxiishortname} & {\wxxishortname}
& {\wxiishortname} & {\wxxishortname}
& {\wxiishortname} & {\wxxishortname}
\\
\midrule
\multicolumn{6}{l}{\emph{\textbf{\uniname}}}
\\
& \emph{\acrnname}
&	10.5	&	9.4	&	10.5	&	9.5	&	14.2	&	14.1	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
\\
& \emph{\wordname}
&	11.9	&	11.1	&	12.2	&	11.3	&	14.7	&	14.6	&	6.2\%	&	3.6\%	&	7.7\%	&	4.1\%	&	43.5\%	&	40.6\% %pg
\\
& \emph{\fnname}
&	11.0	&	10.1	&	10.9	&	10.2	&	14.2	&	14.2	&	2.1\%	&	1.1\%	&	1.9\%	&	1.2\%	&	18.9\%	&	18.9\% %pg
\\
& \emph{\lnname}
&	11.6	&	10.8	&	11.9	&	11.1	&	15.0	&	14.9	&	2.1\%	&	1.2\%	&	2.5\%	&	1.5\%	&	21.8\%	&	20.3\% %pg
\\
& \emph{\filnname}
&	12.6	&	11.7	&	12.9	&	12.1	&	16.3	&	16.2	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	2.1\%	&	1.9\% %pg
\\
& \emph{\fnlnname}
&	12.7	&	11.8	&	12.8	&	12.1	&	16.9	&	16.9	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\% %pg
\\
& \emph{\fsfnlnname}
&	14.1	&	13.3	&	14.4	&	13.7	&	17.2	&	17.1	&	1.0\%	&	\textless1\%	&	1.2\%	&	\textless1\%	&	8.2\%	&	7.7\% %pg
\\
& \emph{\ctryname}
&	9.0	&	9.0	&	8.9	&	8.9	&	9.1	&	9.1	&	93.3\%	&	93.3\%	&	87.1\%	&	87.1\%	&	\textgreater99\%	&	\textgreater99\% %pg
\\
& \emph{\rgnname}
&	14.4	&	13.6	&	14.1	&	13.3	&	17.1	&	17.0	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	\textless1\%	&	5.1\%	&	4.7\% %pg
\\
& \emph{\natlname}
&	8.5	&	8.4	&	8.5	&	8.4	&	8.7	&	8.7	&	70.7\%	&	66.0\%	&	70.7\%	&	66.0\%	&	81.2\%	&	81.2\% %pg
\\\multicolumn{6}{l}{\emph{\textbf{\empname}}}
\\
& \emph{\acrnname}
&	8.2	&	7.8	&	8.1	&	7.7	&	9.6	&	9.6	&	28.7\%	&	21.8\%	&	26.8\%	&	20.3\%	&	75.8\%	&	75.8\% %pg
\\
& \emph{\wordname}
&	10.3	&	9.8	&	10.5	&	9.8	&	11.9	&	11.9	&	25.0\%	&	17.7\%	&	28.7\%	&	17.7\%	&	75.8\%	&	75.8\% %pg
\\
& \emph{\fnname}
&	8.5	&	8.2	&	8.4	&	8.2	&	9.4	&	9.4	&	46.7\%	&	37.9\%	&	43.5\%	&	37.9\%	&	87.1\%	&	87.1\% %pg
\\
& \emph{\lnname}
&	9.2	&	8.8	&	9.1	&	8.7	&	10.4	&	10.4	&	35.4\%	&	26.8\%	&	33.0\%	&	25.0\%	&	81.2\%	&	81.2\% %pg
\\
& \emph{\filnname}
&	11.3	&	10.6	&	11.2	&	10.8	&	13.1	&	13.1	&	9.5\%	&	5.8\%	&	8.8\%	&	6.7\%	&	33.0\%	&	33.0\% %pg
\\
& \emph{\fnlnname}
&	12.7	&	12.0	&	12.4	&	11.7	&	13.6	&	14.3	&	10.2\%	&	6.2\%	&	8.2\%	&	5.1\%	&	18.9\%	&	30.8\% %pg
\\
& \emph{\fsfnlnname}
&	11.3	&	10.9	&	11.2	&	10.9	&	12.2	&	12.2	&	40.6\%	&	30.8\%	&	37.9\%	&	30.8\%	&	75.8\%	&	75.8\% %pg
\\
& \emph{\ctryname}
&	5.8	&	5.7	&	5.8	&	5.7	&	5.8	&	5.8	&	93.3\%	&	87.1\%	&	93.3\%	&	87.1\%	&	93.3\%	&	93.3\% %pg
\\
& \emph{\rgnname}
&	9.3	&	9.0	&	9.1	&	8.9	&	10.0	&	9.9	&	40.6\%	&	33.0\%	&	35.4\%	&	30.8\%	&	66.0\%	&	61.6\% %pg
\\
& \emph{\natlname}
&	5.3	&	5.3	&	5.3	&	5.3	&	5.4	&	5.4	&	93.3\%	&	93.3\%	&	93.3\%	&	93.3\%	&	\textgreater99\%	&	\textgreater99\% %pg
\\
\bottomrule
\end{tabular}


==> tab/tsdicts.tex <==
\begin{tabular}{lrr@{\hspace{3em}}*{1}{rr}}
\toprule
%& & 
%& \multicolumn{2}{c}{\emph{NYT}}
%\\
%\cmidrule(lr){4-5}
\emph{Dict.}
& \emph{Size}
& \emph{$H_{u}(X)$}
& \emph{NYT Occ.}
& \emph{$H^{vr}_{e}(X)$} \\
\midrule
\emph{TSFN} & - & - & - & - \\
\emph{TSLN} & - & - & - & - \\
\emph{TSFILN} & - & - & - & - \\
\emph{TSFIxLN} \\
\emph{\fsfnlnname} & - & - & - & - \\
\emph{TSFNxLN} \\
\bottomrule
\end{tabular}


==> tab/wild-res-2.tex <==
\begin{tabular}{l@{\hspace{-0.005cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}r@{\hspace{0.2cm}}rr}
  \toprule
  Metric              & Name    & Mr      & Ms      & Mrs     & Dr       & FILN    \\
  \midrule
  \textbf{OIG} Total  & 18      & 12      & 11      & 7       & 12       & 16      \\
  Exact Widths        & 2       & 1       & 2       & 0       & 0        & 0       \\
  Exact Matches       & 1       & 1       & 1       & 0       & 0        & 0       \\
  Avg Rank            & 7,953   & 6,947.5 & 9,737   & 804     & 2,074.2  & 860.3   \\
  Med Rank            & 950     & 532.5   & 1,018   & 461     & 1,017.5  & 110.5   \\
  Min Rank            & 6       & 87      & 41      & 29      & 52       & 6       \\
  Max Rank            & 45,189  & 61,436  & 48,347  & 2324    & 8,570    & 4410    \\
  Avg Widths          & 122.4   & 63.67   & 34.55   & 33.29   & 47.33    & 664.94  \\
  Med Widths          & 84      & 34.5    & 24      & 12      & 43       & 277.5   \\
  Min Widths          & 1       & 1       & 1       & 6       & 2        & 8       \\
  Max Widths          & 566     & 308     & 155     & 93      & 113      & 1,928   \\
  Avg Matches         & 182.7   & 219.4   & 125.1   & 258.3   & 172.83   & 4,218   \\
  Med Matches         & 118     & 118     & 66      & 76      & 105      & 1,692   \\
  Min Matches         & 1       & 1       & 1       & 19      & 12       & 42      \\
  Max Matches         & 744     & 1,065   & 426     & 999     & 452      & 12,809  \\
  \midrule
  \textbf{FOIA} Total & 316     & 110     & 105     & 64      & 131      & 266     \\
  Exact Widths        & 12      & 18      & 19      & 6       & 13       & 14      \\
  Exact Matches       & 9       & 4       & 4       & 5       & 3        & 4       \\
  Avg Rank            & 6,554   & 9,536   & 21,315  & 10,483  & 13,018.7 & 7064    \\
  Med Rank            & 737     & 970     & 1,211   & 1,439   & 2,038.5  & 271     \\
  Min Rank            & 1       & 1       & 4       & 7       & 4        & 1       \\
  Max Rank            & \foiaNameMaxRank & 98,099  & 126,018 & 101,737 & 157,234  & 141,140 \\
  Avg Widths          & 97.11   & 54.54   & 57.76   & 45.41   & 50.06    & 439     \\
  Med Widths          & 39      & 13      & 15      & 17      & 9.5      & 58      \\
  Min Widths          & 1       & 1       & 1       & 1       & 1        & 1       \\
  Max Widths          & 1,060   & 651     & 513     & 451     & 493      & 7055    \\
  Avg Matches         & 232.9   & 185.6   & 183.74  & 166.6   & 149      & 2448.7  \\
  Med Matches         & 110     & 42      & 40      & 70      & 28       & 388.5   \\
  Min Matches         & 1       & 1       & 1       & 1       & 1        & 1       \\
  Max Matches         & 2,576   & 1,366   & 1,103   & 1,025   & 1,311    & 29,790  \\
  \bottomrule
\end{tabular}

% for n in names_all mr_surnames ms-surnames mrs_surnames dr_surnames fi_surnames; do echo $n; cat oig_results.txt | grep -v 'NaN' | grep $n | grep -o '.*.json' | sed 's/.'$n'.res,/\n/g' | wc -l; done

% for n in names_all mr_surnames ms-surnames mrs_surnames dr_surnames fi_surnames; do
%   echo "$n";
%   cat oig_results.txt |
%     grep -v 'NaN' |
%     grep $n |
%     cut -f9 |
%     R -q -e 'x <- scan("stdin", what = double()); summary(x);';
% done
%  for n in names_all mr_surnames ms-surnames mrs_surnames dr_surnames; do  cat oig_results.txt  | grep $n | grep -ow 'target.*.json' | sed 's/\.names_all.res,/\n/' | wc -l; done


==> tab/wild-res.tex <==
%\begin{tabular}{l@{\hspace{-3pt}}r@{\hspace{6pt}}r@{\hspace{3pt}}r@{\hspace{3pt}}r|r}
\begin{tabular}{lrr@{\hspace{3pt}}r@{\hspace{3pt}}r|r}
  \toprule
    Metric             & FOIA              & OIG              & DNSA                & rRECAP               & RECAP                     \\
  \midrule
Documents          & 3,145             & \oigNumDocs           & \dnsaNumDocs        & \recapNumDocs        & $\approx10^{7}$           \\
  Pages              & \foiaPg           & \oigPg          & \dnsaPg             & \recapPg             & \numRECAPpages            \\
  % Non-raster Pages &                   &                  &                     &                      & RECAP                     \\
  Redacted PDFs      & 236               & 1255             & \dnsaNumDocsWRedact & \recapNumDocsWRedact & \numRECAPredactionDocs    \\
  %Redacted Pages    & XXX               & XXX              & XXX                 & XXX                  & XXX                       \\
  Redactions         & \foiaMetaRedact & \oigMetaRedact & \dnsaMetaRedact     & \recapMetaRedact     & \numRECAPNameredactions   \\
  \ Unadjusted     & 2,844             & 314              & \unadjDNSA          & \unadjRECAP          & \numRECAPnadj             \\
  \ Adobe OCR      & 3,406             & 1,814            & \ocrDNSA            & \ocrRECAP            & \numRECAPocr              \\
  \ Near Word   & 175               & 114              & \mswDNSANear        & \mswRECAPNear        & \numRECAPNearMSW          \\
  \ Unrec.   & \unrecFOIA &  \unrecOIG         & \unrecDNSA          & \unrecRECAP          & \numRECAPunk              \\
  \ Exact Word     & 4,694             & 455              & \mswDNSAExact       & \mswRECAPExact       & \numRECAPmsw              \\
  Vulnerable       & 711               & 58               & 9                   & 0                    & \numRECAPmsw              \\
  \midrule
    No Matches          & \numFOIAUnmatched & \numOIGUnmatched & 1                  & --                   & N/A                        \\
  Uniq. Matches      & \numFOIAUniq      & \numOIGUniq      & 5                  & --                   & N/A                        \\
  Avg. Matches        & \numFOIAavg       & \numOIGavg       & 393                  & --                   & N/A                        \\
  Med. Matches        & \numFOIAmed       & \numOIGmed       & 1                  & --                   & N/A                        \\
  \bottomrule
\end{tabular}

%   \begin{tabular}{l@{\hskip -3cm}lrrrr}
%     \toprule
%     \multicolumn{2}{l}{}                               & \emph{DNSA}                & \emph{FOIA}                      & \emph{Govt.}          & \emph{RECAP}                                                   \\
%     \midrule
%     \multicolumn{2}{l}{Documents}                      & \dnsaNumDocs               & xxx  & \govtNumDocs          & \recapNumDocs                                                  \\
%     \multicolumn{2}{l}{Pages}                          & \dnsaPg                    & xxx  & \govtPg               & \recapPg                                                       \\
%     \multicolumn{2}{l}{Non-raster pages}               & \dnsaNonRastPg             & xxx  & \govtNonRastPg        & \recapNonRastPg                                                \\
%     \multicolumn{2}{l}{Redacted docs}                  & \dnsaNumDocsWRedact        & xxx  & \govtNumDocsWRedact   & \recapNumDocsWRedact                                           \\
%     \midrule
%     \multicolumn{2}{l}{Redacted text objs.}            & \dnsaMetaRedact            & xxx  & \govtMetaRedact       & \recapMetaRedact                                               \\
%                                                        & Unadjusted                 & xxx  & \unadjFOIA            & \unadjGOVT                            & \unadjRECAP            \\
%                                                        & Adobe OCR                  & xxx  & \ocrFOIA              & \ocrGOVT                              & \ocrRECAP              \\
%                                                        & Exact MS Word (>100 chars) & xxx  & \mswFOIAExact         & \mswGOVTExact                         & \mswRECAPExact         \\
%                                                        & Exact MS Word (<5\% error) & xxx  & \mswFOIAExactFivePerc & \mswGOVTExactFivePerc                 & \mswRECAPExactFivePerc \\
% %    \multicolumn{2}{l}{\ \ Exact 2012}                & \mswDNSAExactTwelve        & xxx  & \mswGOVTExactTwelve   & \mswRECAPExactTwelve                                           \\
% %    \multicolumn{2}{l}{\ \ Exact 2021}                & \mswDNSAExactTwenty        & xxx  & \mswGOVTExactTwenty   & \mswRECAPExactTwenty                                           \\
%                                                        & Near MS Word               & xxx  & \mswFOIANear          & \mswGOVTNear                          & \mswRECAPNear          \\
% %    \multicolumn{2}{l}{\ \ Near 2012}                 & \mswDNSANearTwelve         & xxx  & \mswGOVTNearTwelve    & \mswRECAPNearTwelve                                            \\
% %    \multicolumn{2}{l}{\ \ Near 2021}                 & \mswDNSANearTwenty         & xxx  & \mswGOVTNearTwenty    & \mswRECAPNearTwenty                                            \\
%                                                        & Unrecognized adj.          & xxx  & \unrecFOIA            & \unrecGOVT                            & \unrecRECAP            \\
% %    \multicolumn{2}{l}{\ \ Unknown font}              & \unrecDNSAUnkFont          & xxx  & \unrecGOVTUnkFont     & \unrecRECAPUnkFont                                             \\
% %    \multicolumn{2}{l}{\ \ Known font}                & \unrecDNSAKnwFont          & xxx  & \unrecGOVTKnwFont     & \unrecRECAPKnwFont                                             \\
%     \midrule
%     uncor names\_all                                   &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 42/626 (6.7\%), 19/232 (8.2\%), 0/0   & 0/0, 0/0, 0/0          \\
% uncor mr\_surnames                                     &                            & 1/1 (100.0\%), 0/0, 1/2 (50.0\%) & xxx & 19/296 (6.4\%), 11/122 (9.0\%), 0/0   & 0/0, 0/0, 0/0          \\
% uncor mrs\_surnames                                    &                            & 0/0, 0/0, 0/0                    & xxx & 16/210 (7.6\%), 2/79 (2.5\%), 0/0     & 0/0, 0/0, 0/0          \\
% uncor names\_all\_straight\_pos                        &                            & 1/1 (100.0\%), 0/0, 0/0          & xxx & 7/57 (12.3\%), 2/20 (10.0\%), 0/0     & 0/0, 0/0, 0/0          \\
% uncor names\_all\_curly\_pos                           &                            & 0/0, 0/0, 0/0                    & xxx & 16/218 (7.3\%), 3/83 (3.6\%), 0/0     & 0/0, 0/0, 0/0          \\
% uncor ameng                                            &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 47/604 (7.8\%), 19/227 (8.4\%), 0/0   & 0/0, 0/0, 0/0          \\
% uncor countries                                        &                            & 0/0, 0/0, 1/1 (100.0\%)          & xxx & 81/128 (63.3\%), 33/50 (66.0\%), 0/0  & 0/0, 0/0, 0/0          \\
% uncor demonyms                                         &                            & 0/0, 0/0, 2/2 (100.0\%)          & xxx & 69/98 (70.4\%), 25/30 (83.3\%), 0/0   & 0/0, 0/0, 0/0          \\
% cor names\_all                                         &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 46/460 (10.0\%), 19/152 (12.5\%), 0/0 & 0/0, 0/0, 0/0          \\
% cor mr\_surnames                                       &                            & 1/1 (100.0\%), 0/0, 1/2 (50.0\%) & xxx & 19/249 (7.6\%), 11/90 (12.2\%), 0/0   & 0/0, 0/0, 0/0          \\
% cor mrs\_surnames                                      &                            & 0/0, 0/0, 0/0                    & xxx & 16/190 (8.4\%), 2/70 (2.9\%), 0/0     & 0/0, 0/0, 0/0          \\
% cor names\_all\_straight\_pos                          &                            & 1/1 (100.0\%), 0/0, 0/0          & xxx & 7/57 (12.3\%), 2/20 (10.0\%), 0/0     & 0/0, 0/0, 0/0          \\
% cor names\_all\_curly\_pos                             &                            & 0/0, 0/0, 0/0                    & xxx & 18/168 (10.7\%), 5/52 (9.6\%), 0/0    & 0/0, 0/0, 0/0          \\
% cor names\_all,mr\_surnames                            &                            & 0/2 (0.0\%), 0/0, 0/2 (0.0\%)    & xxx & 48/554 (8.7\%), 22/188 (11.7\%), 0/0  & 0/0, 0/0, 0/0          \\
% cor names\_all,mrs\_surnames                           &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 40/535 (7.5\%), 15/186 (8.1\%), 0/0   & 0/0, 0/0, 0/0          \\
% cor names\_all,names\_all\_straight\_pos               &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 49/488 (10.0\%), 22/162 (13.6\%), 0/0 & 0/0, 0/0, 0/0          \\
% cor names\_all,mr\_surnames,names\_all\_straight\_pos  &                            & 0/2 (0.0\%), 0/0, 0/2 (0.0\%)    & xxx & 51/579 (8.8\%), 24/197 (12.2\%), 0/0  & 0/0, 0/0, 0/0          \\
% cor names\_all,mrs\_surnames,names\_all\_straight\_pos &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 43/557 (7.7\%), 17/194 (8.8\%), 0/0   & 0/0, 0/0, 0/0          \\
% cor names\_all,names\_all\_curly\_pos                  &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 51/524 (9.7\%), 19/176 (10.8\%), 0/0  & 0/0, 0/0, 0/0          \\
% cor names\_all,mr\_surnames,names\_all\_curly\_pos     &                            & 0/2 (0.0\%), 0/0, 0/2 (0.0\%)    & xxx & 49/603 (8.1\%), 22/210 (10.5\%), 0/0  & 0/0, 0/0, 0/0          \\
% cor names\_all,mrs\_surnames,names\_all\_curly\_pos    &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 44/587 (7.5\%), 16/206 (7.8\%), 0/0   & 0/0, 0/0, 0/0          \\
% cor ameng                                              &                            & 0/2 (0.0\%), 0/0, 1/2 (50.0\%)   & xxx & 52/450 (11.6\%), 18/154 (11.7\%), 0/0 & 0/0, 0/0, 0/0          \\
% cor countries                                          &                            & 0/0, 0/0, 1/1 (100.0\%)          & xxx & 81/83 (97.6\%), 30/31 (96.8\%), 0/0   & 0/0, 0/0, 0/0          \\
% cor demonyms                                           &                            & 0/0, 0/0, 2/2 (100.0\%)          & xxx & 76/79 (96.2\%), 25/25 (100.0\%), 0/0  & 0/0, 0/0, 0/0          \\
% \midrule
%     Correlated FN/LNs                                  &                            & \dnsaExactName                   & xxx & \govtExactName                        & \recapExactName        \\
%     FNLN Cases                                         &                            & \dnsaExactName                   & xxx & \govtExactName                        & \recapExactName        \\
%     Matched FNLNs                                      &                            & \dnsaExactName                   & xxx & \govtExactName                        & \recapExactName        \\
%     \midrule
%     Total Exact                                        &                            & \dnsaExactName                   & xxx & \govtExactName                        & \recapExactName        \\
%     True Positive Exact                                &                            & \dnsaExactName                   & xxx & \govtExactName                        & \recapExactName        \\
%     False Positive Exact                               &                            & \dnsaExactName                   & xxx & \govtExactName                        & \recapExactName        \\
%     \bottomrule
%   \end{tabular}


==> tools-scrap.tex <==



Correct deredaction requires a correct positioning scheme model and metadata \emph{integrity}, confidence in the correctness of inferences made about redacted content from PDF metadata.
We therefore measure whether different PDF redaction tools remove or modify redacted and non-redacted positioning information.
To select these tools, we performed web searches for ``PDF redaction tool'', ``redaction tool'' and ``document redaction tool'' and downloaded all redaction tools identifiable from sites in the first five result pages.
Although other redaction tools exist, this sample is representative of PDF redaction's current state.
We classify redaction tools into three categories (Table~\ref{tab:tools}), ordered by descending degrees of metadata integrity:

\paragraph{Full text.}
This redaction category leaks complete redacted content by obscuring the text, e.g. with a black box, but not removing metadata.
Section~\ref{sec:wild} includes a controlled evaluation of our attacks on these \emph{trivial} redactions.
In Section~\ref{sec:ident-weak}, we find U.S. court PDFs contains thousands of trivial redactions.

\paragraph{Width and displacements.}
In this category, ``Width'' indicates the tool preserves redacted contents' width to within one half of a displacement unit.
``Displacements'' indicates the tool preserves non-redacted text positioning metadata.
This classification has one exception: iText aggregates each word's displacements and applies them to the word's successor space glyph.
Although iText leaks more information than unadjusted schemes, we omit this exception's evaluation for simplicity.

\paragraph{Raster width.}
Rasterizing redaction tools remove all text metadata by converting the document into an image.
At 600 DPI, this quantizes displacements to 10 unit boundaries, reducing deredaction attacks' efficacy.
Moreover, the rasterizer may change the glyphs' positioning during conversion.
Prior work has assumed the opposite, reporting positive results for matching raster redactions (Section~\ref{sec:related}).
These misleading results not only ignore the rasterizer, but are incorrect for any PDF with displacements.
Recall that the efficacy of proportional font deredaction depends on each word having a unique width.
We found dictionaries of words and names create an almost \emph{continuous} function $f(w)=y$, where $w$ is width and $y$ is a number of words with that width.
Imprecision at the level of single displacement leads to a different redacted content match.
Prior work's conflation of TTF or PDF widths with printed character widths is both imprecise and misleading.

For each technology in Table~\ref{tab:tools} we created a PDF with text from a random NYT article (Section~\ref{sec:synth}) in Times New Roman 12pt font with all positioning features identified by previous sections.
Of the redaction tools we studied, leaking width and displacement information was the most common behavior.
In Sections~\ref{sec:eval} and~\ref{sec:wild} we attack this ``secure'' redaction category.

For completeness we note redacted characters can leak via other PDF metadata.
Glyph mappings (CID, Width, TTF) leak information when mapped characters are a subset of the complete alphabet.
That is, if the letter ``A'' occurred in text metadata prior to redaction but ``b'' never occured, ``A'' may be present in glyph maps and not ``b''.
Therefore, if ``A'' occurred only in redacted content, the glyph maps leak information.
\maxray\ uses these leaks during deredaction.
\emph{Extended metadata} information leaks also exist, such as PDF annotations.
We found only rasterizing redaction tools removed this metadata.

==> wild-scrap.tex <==

XXX

We attacked names occuring as \emph{the first redaction on the line}, to avoid dependencies between results.

\subsubsection{Hybrid-Synthetic}
The first is \numRECAPPDFs\ PDF documents from the entire CourtListener (RECAP) document corpus.
RECAP is a free legal research website that mirrors legal documents obtained from PACER, a paid service for accessing United States court documents.
We combed these PDFs for trivial redactions, returning \numRECAPredactions\ redacted words in total, including social security numbers and other sensitive information.
We then located names inside this set of redactions matching our dictionaries of first names and surnames from Section~\ref{sec:synth}, including titles (Mr., Mrs., Ms., and Dr.) and first initial, last name combinations, resulting in the \numRECAPNameredactions\ name redactions given in Table~\ref{tab:wildres}.
While the number of name redactions is small relative to the total number of documents, ($\alpha$) the expected number of redacted documents among the whole population of court documents is small and ($\beta$) we rely on finding ``naive'' redactions, which are trivially broken and require a supreme degree of negligence (or a small degree of malintent) to produce.

We found redacted names within this set of redactions, correctly redacted them, and then used knowledge of the ground truth (the redacted name) to validate (blindly) the efficacy of our techniques (Section~\ref{sec:hybrid-synth}).
For these attacks we used a combined dictionary that includes all first names and surnames, \nameDictSize\ names in total.

\subsubsection{Nonsynthetic}
The second corpus contains four sources of documents:
\begin{enumerate}
\item A large set of publically available Freedom of Information Act (FOIA) documents~\cite{}. The FOIA allows for public access to government documents on request to US local and national governments, with some restrictions~\cite{}.
\item All publically available Office of the Inspector General (OIG) investigation reports~\cite{}. The OIG is an oversight branch of the US government aimed at preventing unlawful or inefficient operation.
\item All Digital National Security Archive (DNSA) documents produced after 2010. The DNSA is a set of historically important documents relating to US national security curated by scholars in the field~\cite{}.
\item All RECAP documents for which the word ``redact'' occurs somewhere in the document's metadata (denoted rRECAP).
\end{enumerate}

These corpora were not previously available; data and associated scripts are released alongside our source code.
For this second set of documents we had no ground truth; we tagged redactions as names manually from the set of all redactions with a size less than 2.1cm and greater than 0.7cm.
This resulted in \totalNonSynthNames\ names from a set of \numNonSynthRedactions\ redactions matching the Word adjustment scheme.
An analysis of unadjusted redactions was unnecessary given the pessimistic results of Section~\ref{sec:hybrid-synth}.
We found that \emph{none} of the rRECAP redactions we discovered contained guessable names; this is a negative result that indicates that more advanced techniques for redaction location will be necessary for handling extremely large dataset of PDF files (Section~\ref{sec:disc}).
Nonetheless we attack the remaining names, demonstrating the extent to which deredaction can be leveraged in the wild, in Section~\ref{sec:nonsynth}.
For these attacks we use the same \nameDictSize\ name dictionary we used to attack the Hybrid-Synthetic cases.

\subsection{Location}

The first step in assessing the vulnerability of redactions is locating redactions.
For this, we divide redactions into \emph{trivial}, and \emph{nontrivial} categories.
Trivial redactions occur when the text underneath the redaction can be highlighted and copy-pasted using a standard PDF reader.
Nontrivial redactions occur when the text underneath the redaction is removed and must be inferred using residual information leakages present elsewhere in the document (Section~\ref{sec:pdftext}).

We wrote a location algorithm for trivial redactions based upon a two-pass scheme, where the first pass checks for a rectangle drawn in the PDF intersecting with the coordinates of a text object on the page.
If this check passes, we generate two PNGs from the PDF document, one with text objects and the other without, and then, iterating over the coordinates of each word, we check whether the pixel color values do not change across both PNGs: this indicates the words in question were not visible in the original PDF document.

Locating nontrivial redactions required a different, more expensive redaction location strategy: we generate a PNG from the PDF document and attempting to ``walk'' the boundaries of boxes placed in-between words on the page.
Unavoidable computational costs involved in an effective location algorithm prevented us from running on the entire RECAP corpus: we discuss the costs and challenges of large corpora further in Section~\ref{sec:disc}.
We compared this algorithm to one developed by Timothy B. Lee which records graphics state draw commands~\cite{}, finding that there are fewer false positives and more vulnerable width-based redactions are flagged (we also found it equivalent to results attained by manual analysis; see Appendix Table~\ref{tab:redactfind}).



\subsubsection{Dictionary Selection}\label{sec:dict-select}

We did not choose to attack names by chance: to determine the most common redaction type in these documents we conducted a random sample of 100 redactions from the population and manually tagged their dictionary type, resulting in the following distribution:

\begin{center}
\begin{tabular}{c|c|c|c|c}
  Word & Too Long & Name & Number & Pronoun \\
  2 & 26  & 52 & 17 & 3 \\
\end{tabular}
\end{center}

Thus, while the set of dictionaries from Section~\ref{sec:synth} is comprehensive, it is not necessary reflective of population statistics.
Redactions are most commonly names (of some length).
We note, however, that names of regions were still important for attacking several redactions in one of our case studies (Section~\ref{sec:snowden}).

\subsection{Scheme Identification}

\begin{table}
  \centering
  \caption{Glyph adjustment schemes identified in pages containing text from the redacted document corpora. The * indicates the hybrid-synthetic reduction from \numRECAPredactions\ word-redactions to name redactions.}
  \label{tab:wildres}
  \include{tab/wild-res}
\end{table}

Once a set of redactions are located, we identify the displacement scheme used to generate the PDF document (Section~\ref{sec:pdftext}).
In determining the adjustment scheme of trivial redactions, we use the ground truth for the line in question to match the correct scheme.
For determining the adjustment scheme of nontrivial redactions, we model the expected scheme and look for greater than 100 characters on the page that abide by the scheme's metrics.
This is counted per-line: an entire line is classified and if it matches, then the characters of that line are counted toward the scheme's score.
This is done to handle unimplemented cases of formatting that will affect glyph displacements\footnote{Such as footnotes.} for a subset of the lines on a page.
For each of the MS Word cases, we ensure that the prefix of the line prior to redaction exactly matches the MS Word model.
We include fixes for the \emph{i,l} displacement scheme discussed in Section~\ref{sec:snowden} in our set of exact MS Word displacement scheme matches for completeness.\footnote{We ensure the page contains both \emph{i} and \emph{l} if classified as needing this fix.}
Table~\ref{tab:wildres} gives our results.

We find a large number of unrecognized displacement schemes as we do not consider multiple applied transforms, that is, a PDF run through OCR and then opened in Microsoft Word.
In the case of the RECAP hybrid-synthetic dataset, a random sample of 20 redacted documents found that all of the unrecognized schemes were either due to an unrecognized unicode character or (mostly) due to specific document layout templates used by US courts, typically implemented in Microsoft Word, but needing additional, idiosyncratic scheme modeling (Section~\ref{sec:word-templates}).
Similar problems arise for documents created in email clients, spreadsheets, and templating software; we discuss these more complex flows in Section~\ref{sec:flow-disc} and give an example of two such cases in Sections~\ref{sec:snowden} and \ref{sec:manafort}.
The unrecognized adjustment schemes reported in Table~\ref{tab:wildres} are sufficiently distant from our Microsoft Word models: we give a notion of this distance with the \emph{near Word} case: we took the $L_{1}$ distance from the expected Word text showing operator and thresholded a maximum distance of 10 units for every 100 characters.

Finally, we note that for all cases (both unadjusted and Word), we attack each redaction at a page granularity, correlating the results for redactions that appear to be the same content (the same name redacted multiple times).

\section{Hybrid Synthetic Evaluation}\label{sec:hybrid-synth}

In this section we combed our first corpus, the entirety of RECAP, for trivially redacted names (highlighted black but not removed from the PDF).
We then correctly redacted the sets of \numRECAPmsw\ names matching Word adjusment schemes and \numRECAPnadj\ names matching an unadjusted scheme and used knowledge of the ground truth (the redacted name) to validate (blindly) the efficacy of our techniques.
This also allowed us to examine how well statistical ranking works in resolving cases where deredaction returns more than one possible name.

\subsection{Results}

\begin{table}
  \centering
  \caption{Efficacy of deredaction inside a corpus of court documents for which the ground truth is known. Resultant names weighted according to their popularity in the US census. The ``rank'' here refers to the probability of the name occuring in the US census relative to the other names that were exactly matched.}
  \label{tab:hybrid-synth-res}
  \include{tab/hybrid-synth-res}
\end{table}

Table~\ref{tab:hybrid-synth-res} reports the results for attacking the Word redactions.
Note that the number of rows here is smaller than \numRECAPmsw\ due to cross-context information correlation (Section~\ref{sec:ms-word}).
For all of the results, \maxray\ correctly deredacted the ground truth name, but not always as an unique match.
Here, \emph{Widths} refers to unique matches for the font metrics used by the adjustment algorithm; that is, in one case we got a \emph{perfect} reduction for the guessed name as all other exactly matching names were indistinguishable with respect to their effect on the context of the Word algorithm.
\emph{Widths} is in contrast to \emph{Matches}, which reports the number of names matching the target from our dictionary of \nameDictSize.
With each of these results we rank the correct name by popularity the US census~\cite{} with respect to other Matches, e.g. a rank of 1 indicates the name is the most popular among the exactly matching guesses.
$p_{coll}$ gives the sum of the probabilities of the set of incorrect Matches: the population of the census with that set of names divided by the total population.
The z-score for $p_{name}$ with respect to the other Matches is given to provide a sense of the distribution.
We also include a measure of the number of names it is necessary to select at random from our corpus of names until the likelihood of having two Matches is greater than 5\%, where the correct name is guaranteed to be included:
$$\sum_{k = 1}^{n}\binom{n}{k}(\frac{p_{coll}}{(1 - p_{name})})^{k}(\frac{1 - p_{name} - p_{coll}}{(1 - p_{name})})^{n-k}$$
We find on average, a shortlist of \avgShortlist\ names has no more than a 5\% chance of having a colliding Match, with an average 800-fold reduction of the original dictionary to \avgNumNames, where the correct name is on average \avgStdDevRECAPName\ standard deviations above the mean US census popularity of other Matches.

In attacking unadjusted redactions (labeled ``nadj.'' in the table), results were pessimistic: the average match set size was far greater than Word and no redaction attacked resolved to an exact match.
However, these methods are still effective if the size of the dictionary used is small (Section~\ref{sec:manafort}).

\section{Nonsynthetic Evaluation}\label{sec:nonsynth}

\begin{table}
  \centering
  \caption{Matching results for the set of names that were extracted out of the redacted document corpora. The FILN column indicates results for matching first initial, last name pairs; other columns correspond to single-word names and names prefixed by the given title.}
  \label{tab:wildres2}
  \include{tab/wild-res-2}
\end{table}

In this section we explore how well deredaction generalizes to an uncontrolled setting: redacted documents occuring in the wild.
We focus our attack on documents of public interest (FOIA) and documents relating to government investigations (OIG), finding that historically important and court document redactions are sparse (this is resolved by targeting specific, known cases, see Sections~\ref{sec:epstein} and~\ref{sec:snowden}).
We attack, in particular, \numFOIANamesAttacked\ names from requested FOIA documents, and \numOIGNamesAttacked\ names from OIG investigation reports.
We note that \numOIGUnmatched\ of the OIG cases and \numFOIAUnmatched\ FOIA cases we examined, we were unable to find any exact match; this is due to a number of factors, including typos, alternative formatting of the name (placing it outside of our dictionary), and use of a FNLN pair (Section~\ref{sec:disc-dict-gen}).
For a few of the documents for which it was possible to determine the ground truth redacted names, we were able to manually validate our technique returned the correct name (after the attack was performed).
We omit discussion of these results here, choosing to analyze specific \emph{cases} of deredaction more comprehensively in the studies of Section~\ref{sec:cases}.

\subsection{Results}

Table~\ref{tab:wildres2} reports our results.
First, we note that some redactions contribute to the values of multiple columns: i.e. there are cases were a single word name will match a redaction as well as a shorter name prefixed by a title.
Where it was possible to resolve this ambiguity, we did so manually, but this was not always possible based upon the context of the document.
Determining an \emph{exact} match occurs with a frequency of 3\%, close to the predictions provided by Table~\ref{tab:nyt10}, with a slightly lower success rate due to a smaller amount of information leaked in font sizes greater than 10pt.
It is also more apparent here that the set of \emph{width classes} is quite small compared to the total number of classes for the dictionary used.
An analysis of TNR, Calibri and Arial in 10, 11, and 12 point font reveal the following statistics for the number of width classes in our \nameDictSize\ name dictionary:

\begin{center}
\begin{tabular}{c|c|c|c}
  Min  &  Median  &  Mean  &  Max \\
  68,876 &   109,766 & 135,819 & 214,690 \\
\end{tabular} 
\end{center}

That is, the ratio of the averages of names to matches is \ratioNamesToMatches, while the ratio of dictionary width classes to width matches is \ratioWidthClassesToWidths, more than double the reduction over names alone.
From these results, we can conclude the techniques presented in this paper are both practicable and circumstances for their use are common enough to warrant attention.
In the next section we demonstrate the flexibility of these attacks by deredacting targeted documents of public interest.

% We studied \numWildCorpora\ corpora of redacted text documents:
% 
% % https://nsarchive.gwu.edu/digital-national-security-archive
% \paragraph{DNSA.} Digital National Security Archives is a collection of more than 100,000 declassified records documenting historic U.S. policy decisions curated by scholars.\cite{} We downloaded all DNSA documents that were produced after 2010, including the Snowden case files, one of which is included in Section~\ref{sec:snowden}.
% % https://foiaonline.gov/foiaonline/action/public/home
% \paragraph{FOIA.} The Freedom of Information Act is a law which upon request requires the United States government to either fully or partially disclose documents. We searched foiaonline.gov for the term ``redacted'' and downloaded all returned documents.
% % https://governmentattic.org/
% \paragraph{Gov. Attic.} The Government Attic is an independently run FOIA archive that includes documents of note returned from FOIA requests. We downloaded all the documents from this site and removed duplicates of our previously-scraped FOIA documents.
% \paragraph{PACER/RECAP.} Public Access to Court Electronic Records (PACER) is a service that provides electronic access to US Federal court documents. Unfortunately, while PACER documents are public, access to PACER is not free. The Free Law Project hosts a subset of PACER documents uploaded by volunteers through its RECAP archive. We searched RECAP for the term ``redacted'' and downloaded all returned documents.
% 
% \paragraph{Redaction Location}
% To locate redacted text in the PDF documents from these corpora, we use the following ``Box'' algorithm (released with our source code): 
% 
% \begin{itemize}
%   \item Remove all text showing operators from PDF and convert to a normalized, depth 8 grayscale, 300 DPI ppm.
%   \item Parse the original PDF for the bounding boxes of large spaces between text showing operators on the same line
%   \item Walk from the left boundary, vertical center of the bounding box rightward, looking for a change in color
%   \item If a change is encountered walk the outer boundary of the color and find the rectangle that fits this boundary
%   \item Check that this rectangle is of sufficient width (0.5 of the ``large shift'' and within the bounds of the shift)
% \end{itemize}
% 
% To validate the algorithm described above, we drew a sample of \numWildLocSample\ pages from the corpora and compared the above algorithm against the algorithm described by one of the creators of RECAP, Timothy B. Lee, for locating redactions~\cite{}.\footnote{For space we leave details of Lee's algorithm out. Interested readers may check the cited article: we acquired the code from Mr. Lee himself.}
% Table~\ref{tab:redactfind} summarizes our results.
% In order to provide an honest evaluation, we classified redactions into ``easy'' and ``hard'' categories with the latter being redactions of an entire line of text, the start of a line, or the end of a line.
% Starts and ends are labeled ``hard'' to ensure the accuracy of our results: we avoid interpolating boundary information from the rest of the page.
% We also labeled whether the document contained vector metadata and classify any redactions over rasterized content \emph{raster redactions} (neither algorithm handles rasters).
% Using the Box algorithm, we then were able to identify \totMetaRedact\ instances of redaction across \totNumDocsWRedact\ documents comprising a total of \totNumPagesWRedact\ pages (Table~\ref{tab:wildres}).

% \subsection{Identifying Positioning Scheme}
% \label{sec:schemeid}
% 
% \subsection{Attacking Wild Documents}
% 
% We then attacked the \numWildTotalVuln\ MS Word redactions above with dictionaries of potential words blindly.
% We give our results in Table~\ref{tab:wildres}.
% We then went through the attacked pages for which we had non-exact matches by hand and performed an \emph{intersection} of results for redactions we inferred to be of the same content.
% Correlating the different instances of information leakage in this manner allowed us to get XXX additional exact matches for redacted content that would have otherwise not been possible, one ``benefit'' of the MS Word adjustment model.
% 
% We then took the set of one-word names we were able to exactly guess and looked for firstname, lastname cases on the same pages that \emph{became} vulnerable as a result of our guess for one half of the name.
% This resulted in XXX guessable firstname, lastname cases in total, XXX we were able to guess exactly.
% As a final validation set, we took the pages for which we had exact match results and googled for information relating to the original document: we were able to confirm we correctly deredacted the name in XXX of these cases.
% 
% For completeness, we note that while we consider exact matches to be our strongest result, the overall reduction in the space of possible names was often quite large.
% We give a listing of these reductions and in Appendix~\ref{}.

% \subsection{Attacking Wild Documents}

% We attack redactions by using the existence of an exact match as a halting condition.
% If no exact match for the default set of dictionaries is found, we first try unedited dictionaries with premodifiers, then we apply one edit to each of the $n$ positions of each guess, and then if no match is found after these two attempts, we stop guessing.
% Even though in these cases we have not discovered the exact ground truth of the redaction, we have now effectively \emph{ruled out} potentially millions of possibilities.
% 
% With vulnerable redactions identified, we then located 100 redactions for which we could determine a likely dictionary based upon context (50 exact MS Word cases and 50 Adobe OCR cases, and attempted to automatically guess the redacted context.
% XXX of these cases had exact matches for redacted text.
% \note{report other stats.}
% \subsection{Validation}
% 
% For the few cases where we had exact matches, we attempted to validate that our guess for the content was correct by looking up details about the document online.
% We found that for all of our exact matches we were exactly correct at guessing the redacted content, and were able to validate this independently of the guessing process.

% Because the schemes we study are absolutely predictive, \maxray's only failure mode is scheme misclassification.
% For example, a scheme may look fixed per-character for all non-redacted text, with a counterexample in the redacted portion of the text, with no information remaining in the document to indicate an error.
% This particular case is indistinguishable from a perfect counterexample-free case, and there is no hope of handing it (just like there is no hope of knowing \emph{with complete certainty} that you understand this sentence).
% 
% We only consider cases with either no counterexamples or manually explainable counterexamples.
% Counterexamples are easily identified: any line not matching expected displacements exactly.
% For the fixed per-character model, counterexample identification is more complex because the model can adapt to the scheme of the page (Section~\ref{sec:flows})
% 
% 
% 
% Thus, we introduce two pessimistic, worst-case \emph{parts count} reliability predictions~\cite{nukeHandbook}.
% In Fixed Per-Character scheme classification, we assume we are able to classify one line (if at least one fixed per-character line exists) and no more than one line, then we take the worst-case model over all lines.
% This model provides the \emph{maximum} number of counter-examples to a \emph{minimal} Fixed Per-Character positioning scheme.
% If no line in the document can be \emph{honestly} used to bootstrap such a scheme,
% 
% By sorting 
% Any more pessimistic of a model would 
% The difference in the number of lines classified as belonging to the scheme by this model and the number of lines in the document tells us whether any counter-examples (failures) to the model exist.
% 
% This is a severe underestimate of documents conforming to this scheme, 
% 
% To determine the safety of the Word Save-as-PDF scheme, we compute the L1 distance from the modeled displacements for each glyph to the actual displacements.
% We then count the number of lines for which the L1 distance is zero as ``lines classified'' and compare this to the total number of lines.
% For the redacted line in question, we ensure the prefix of the line, prior to the redaction, has an L1 distance of 0 as well.
